Auto-Pipeline: Synthesizing Complex Data Pipelines By-Target Using Reinforcement Learning and Search

Recent work has made significant progress in helping users to automate single data preparation steps, such as string-transformations and table-manipulation operators (e.g., Join, GroupBy, Pivot, etc.). We in this work propose to automate multiple such steps end-to-end, by synthesizing complex data pipelines with both string transformations and table-manipulation operators. We propose a novel "by-target" paradigm that allows users to easily specify the desired pipeline, which is a significant departure from the traditional by-example paradigm. Using by-target, users would provide input tables (e.g., csv or json files), and point us to a "target table" (e.g., an existing database table or BI dashboard) to demonstrate how the output from the desired pipeline would schematically "look like". While the problem is seemingly underspecified, our unique insight is that implicit table constraints such as FDs and keys can be exploited to significantly constrain the space to make the problem tractable. We develop an Auto-Pipeline system that learns to synthesize pipelines using reinforcement learning and search. Experiments on large numbers of real pipelines crawled from GitHub suggest that Auto-Pipeline can successfully synthesize 60-70% of these complex pipelines with up to 10 steps.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $< | sed 's/^%\\citestyle{acmauthoryear}/\\citestyle{acmauthoryear}/'      > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.


==> acmart-master/acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $< | sed 's/^%\\citestyle{acmauthoryear}/\\citestyle{acmauthoryear}/'      > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> acmart-master/acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.


==> algorithm-search_-_orig_-_junwen.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Search-based Auto-Pipeline}
\label{sec:algo}
We are now ready to describe our synthesis algorithm.
We will start with a search-based synthesis \sjs{} in this section,
before describing a learning-based alternative in the next section.


\subsection{A High-level Overview}
\label{sec:algo_overview}

As we describe in Section~\ref{sec:sketch}, 
at a very high level the synthesis process can
be seen as traversing a large search graph
shown in Figure~\ref{fig:synthesis-sketch}.
Because each node corresponds to a partial-pipeline,
and each edge corresponds to the act of
adding one operator, each node $d$-steps away from the
start-node would naturally correspond to a partial-pipeline 
with $d$-operators/steps. 
According to the PMPS formulation, our end goal
is to find pipelines that  (1) have high probabilities
(based on joint operator likelihood); and 
(2) satisfy all FD/Key/column-map constraints. 

Given the large search graph, it is nature 
to explore only the ``promising'' parts of the graph.
We first describe such a strategy in a meta-level synthesis algorithm
shown in Algorithm~\ref{algo:meta} below, which uses a form of 
local beam search~\cite{ow1988filtered}.

\begin{algorithm}[H]
  \caption{A meta-level synthesis algorithm}
  \label{algo:meta}
\begin{small}
  \begin{algorithmic}[1]
  \State {\bf Synthesis}{($\widehat{\mathbf{T}}^{in}, T^{tgt}, \mathbf{O}$)}
  \State $depth \gets 0, candidates \gets \emptyset$
  \State $S_{depth} \gets \{empty()\}$  \Comment{$\#$initialize an empty pipeline}  \label{line:meta_step_0}
  \While{$depth < maxDepth$} \label{line:meta_loop}
    \State{$depth \gets depth + 1 $}
    \ForEach{($ppl \in \mathcal S_{depth-1}$, $O \in \mathbf{O}$)}
      \State{$S_{depth} \gets S_{depth} \cup \textsf{AddOneStep}(ppl, O)$} \label{line:meta_add_one}
    \EndFor
    \State{$S_{depth} \gets \textsf{GetPromisingTopK}(S_{depth}, T^{tgt})$}  \label{line:meta_promising}
    \State{$candidates \gets candidates \cup \textsf{VerifyCands}(S_{depth}, T^{tgt})$}  \label{line:meta_verify}
  \EndWhile
  \State{return $\textsf{GetFinalTopK}(candidates)$} \label{line:meta_return}
  \end{algorithmic}
\end{small}
  \end{algorithm}


Algorithm~\ref{algo:meta} starts
by initializing $depth=0$ to indicate that we are
at the start-node in Figure~\ref{fig:synthesis-sketch}.
Variable $candidates$ stores all ``valid'' pipelines
that satisfy the constraints 
(Equation~\eqref{eqn:fd}-\eqref{eqn:map}), and is
initialized as an empty set.
Variable $S_{depth}$ corresponds to a
set of pipelines with $depth$-steps that are being  
actively explored, and at line~\ref{line:meta_step_0} we initialize it 
to a single placeholder empty-pipeline, since we are at the
start-node.

From line~\ref{line:meta_loop}, 
we iteratively visit nodes that are $depth = \{1, 2, \ldots\}$
steps away from the start-node, which is equivalent
to exploring all pipelines with $depth = \{1, 2, \ldots\}$ operators,  respectively.   As we increment $depth$ in our exploration,
we take all active pipelines from the previous step, or $S_{depth-1}$,
and invoke \textsf{AddOneStep}($ppl, O$) in line~\ref{line:meta_add_one},
which expand each partial pipeline $ppl \in S_{depth-1}$ using one
additional operator $O \in \mathbf{O}$. 
These resulting pipelines with $depth$-step are then
saved into $S_{depth}$.  
Because we cannot exhaustively explore all 
possible nodes/partial-pipelines due to the 
size of the graph, at line~\ref{line:meta_promising}, 
we select top-K most promising partial-pipelines 
from the current $S_{depth}$ by invoking \textsf{GetPromisingTopK}().
We then check these top-K promising pipelines using \textsf{VerifyCand}(),
and mark the ones that satisfy all constraints as candidates
(line~\ref{line:meta_verify}). This marks the end of one iteration
in which we explore promising $depth$-step 
pipelines, by expanding all $(depth-1)$-step promising pipelines 
with one additional operator.

The loop line~\ref{line:meta_loop} continues, as we increment
$depth$ and visit longer pipelines, until we find 
enough number of valid candidates, or we reach the maximum
depth allowed, at which point we return the final 
top-K candidate pipelines
by invoking \textsf{GetFinalTopK}() (line~\ref{line:meta_return}). 

\textbf{Discussion.} While we sketch out the
overall steps of our synthesis in Algorithm~\ref{algo:meta},
there are a few sub-routines that are not yet fully described:
\begin{itemize} % produces lots of vertical space
\item \textsf{AddOneStep()} expands a partial pipeline 
$ppl$ using one additional operator $O \in \mathbf{O}$;
\item \textsf{VerifyCands()} checks whether pipelines
satisfy PMPS constraints, and if so marks them as final candidates;
\item \textsf{GetPromisingTopK()} selects the most promising
top-K pipelines from all $depth$-step pipelines;
\item \textsf{GetFinalTopK()} reranks all candidate
pipelines (which are valid solutions as they satisfy PMPS
constraints), and returns a final
ranked list of synthesized pipelines.
\end{itemize}
 
We should highlight that the last two sub-routines 
\textsf{GetPromisingTopK()} and
\textsf{GetFinalTopK()} are the most critical to \sj{} 
we study in this work --
the design of these two modules ensure 
that we can efficiently search the relevant/promising
parts of the graph to ultimately synthesize pipelines successfully.
In the next section, we 
will describe a search-based strategy to instantiate
these two sub-routines, which is at
the core of \sjs. We will later describe a learning-based alternative
to instantiate these two sub-routines in Section~\ref{sec:learning},
which makes Algorithm~\ref{algo:meta} \sjsl{} and \sjrl{}.



The first two sub-routines, \textsf{AddOneStep()} and 
\textsf{VerifyCands()} are reasonably straightforward on the other hand --
\textsf{AddOneStep()} add one additional step
in partial pipelines by leveraging prior work that predicts
most likely parameters for single-operators 
(AutoSuggest~\cite{auto-suggest}), 
while \textsf{VerifyCands()} checks the satisfaction of PMPS constraint 
by performing standard FD/Key-discovery 
(\cite{buranosky2018fdtool, papenbrock2015functional}) and
column-mapping (\cite{rahm2001survey}).
We will describe these two sub-routines in Section~\ref{} 
and~\ref{}, respectively.


\subsection{Overview} 
This section will introduce our synthesis algorithm (Algorithm~\ref{algo:main_syn}).
Given an a set of input tables $\widehat{\mathbf{T}}^{in}$,  target output $T^{tgt}$, and 
a search width W, the \texttt{Synthesis} alogrithm will firstly normalize the target 
output and generate a set of candidate pipelines through beam search. For each depth,
the algorithm explore the partial pipelines by one step as 
shown in Line~\ref*{line:one_step}. And then it keeps the  W most 
 promising partial pipelines (Line~\ref{line:filter}) for further search.
 At the same time, it select the partial pipelines which is candidate and
 add them to the results set \textit{ppls} (Line~\ref{line:select_candi}). A pipeline
is a candidate pipeline if it meets three requirements, firstly, all the input tables
contribute to the final result, secondly, every column of the target output table can 
be mapped to a column in the final output table of the pipeline, lastly, the FD/Key constraints in the target output table are covered over 90\% in the
pipeline output table. We will introduce the way we compute the column correspondence and 
FD/Key constraints mapping in Section~\ref{subsection:diversity}.
After the results set is not empty for the first time, we record the length 
of the shortest candidate pipelines \textit{minD} (Line~\ref{line:set_minD}), the search algorithm will continue explore
until the difference of the depth and shortest length \textit{minD} exceeds predefined threshold. 
The candidate pipelines will then go through last step tuning and string transformations
and be returned to users after ranking, and the default ranking parameter is 
the joint operator probability.

\begin{algorithm}[H]
  \caption{Main Synthesis Algorithm}
  \label{algo:main_syn}
{\color{blue}$\#$ Input: input tables $\widehat{\mathbf{T}}^{in}$, target output $T^{tgt}$, width W}

{\color{blue}$\#$ Output: pipelines with similar target schema}

  \begin{algorithmic}[1]
  \Procedure{Synthesis}{$\widehat{\mathbf{T}}^{in}, T^{tgt}, W$}
  \State OutputNormalization($\widehat{\mathbf{T}}^{in}, T^{tgt}$)
  \State $S_p \gets [PPL()]$  {\color{blue}{$\#$initialize an empty pipeline}}
  \State $ppls \gets \emptyset, depth \gets 1, minD \gets None$
  \While{$len(S_p) > 0 \land depth - minD < threshold$}
    \State $S_p' \gets \emptyset $
    \ForEach{$p \in \mathcal S_p$}
      \State{$S_p'\gets S_p' \cup SynthesisOneStep(p, \widehat{\mathbf{T}}^{in}, T^{tgt})$}\label{line:one_step}
    \EndFor
    \State{$S_p \gets GetTop(S_p', W)$} \label{line:filter}
    \State{$ppls \gets ppls \cup \{p\: |\: p\: \in \mathcal S_p \land isCandidate(p, T^{tgt})\}$}\label{line:select_candi}
    \If{$len(ppls) > 0 \land minD == None $}
      \State{$minD \gets depth$} \label{line:set_minD}
    \EndIf
    \State{$S_p \gets \{p\: |\: p\: \in \mathcal S_p \land p \not\in ppls\}$}
    \State{$depth \gets depth + 1 $}
  \EndWhile
  \State{$ppls \gets LastStepTuning(ppls)$}
  \State{$ppls \gets StringTransformation(ppls)$}
  \State{return $Rank(ppls)$}
  
  \EndProcedure
  
  \end{algorithmic}
  \end{algorithm}

\subsection{Output Normalization}

Our algorithm assumes that the target output table is a well-normalized table, which is to say that the 
other than the last step, no Pivot operator is involved. So for the output which 
looks like generating from a Pivot operator, we need to normalize it as shown in 
Algorithm~\ref*{algo:normalization}. 
We firstly check whether the columns in output table $T^{tgt}$ overlaps with the column value 
in input tables. If so and the number of overlapped columns 
exceeds 3 or the ratio exceeds 50\%, we assume the output is produced through a Pivot 
operation. We then predict the Pivot parameters using the single step predictor on 
the output table $T^{tgt}$ and apply Pivot operator on  $T^{tgt}$ using the predicted 
parameters.

\begin{algorithm}[H]
  \caption{Output Normalization Algorithm}
  \label{algo:normalization}
{\color{blue}$\#$ Input: input tables $\widehat{\mathbf{T}}^{in}$, target output $T^{tgt}$}

{\color{blue}$\#$ Output: normalized output}

  \begin{algorithmic}[1]
  \Procedure{OutputNormalization}{$\widehat{\mathbf{T}}^{in}, T^{tgt}, K$}
  \ForEach{$T \in \widehat{\mathbf{T}}^{in}$}
  \ForEach{$col \in T$}
    \State{$overlap = len(T[col] \cap T^{tgt}.columns)$}\label{line:overlap}
    \State{$ratio \gets overlap/len(T^{tgt}.columns)$}
    \If{$overlap > 3 \lor ratio > 0.5 $}
      \State{$param = predict(T^{tgt},\:Pivot)$} \label{line:normalize}
      \State{$T^{tgt} \gets Pivot(T^{tgt},\:param)$}
      \State{return $T^{tgt}$}
    \EndIf
  \EndFor
  \EndFor
  \EndProcedure
  
  \end{algorithmic}
  \end{algorithm}

\subsection{Single Step Synthesis}
Algorithm~\ref{algo:single_step_synthesis} shows how we synthesize single
step for a given partial pipeline. For the input tables and intermediate output tables 
generated from previous steps, we filter out them by checking 
whether they have been used in the previous steps (Line~\ref{line:check_used}).

For each one of the filtered tables, we predict the Top K GroupBy 
parameters (Line~\ref{line:loop_groupby}).
For any two of the filtered tables, we predict the Top K parameters for both
Join and Union operator. All the generated step will be used to extend the 
current partial pipeline by one step separately.


\begin{algorithm}[h]
  \caption{Single Step Synthesis}
  \label{algo:single_step_synthesis}
{\color{blue}$\#$ Input: input tables $\widehat{\mathbf{T}}^{in}$, target output $T^{tgt}$, pipeline p}

{\color{blue}$\#$ Output: a set of pipelines with one more step}

  \begin{algorithmic}[1]
  \Procedure{SynthesisOneStep}{$\widehat{\mathbf{T}}^{in}, T^{tgt}, K$}
  \State{$S_t \gets \widehat{\mathbf{T}}^{in} + \{s.output\: |\: s\: \in\: p.steps\}$}
  \State{$S_t \gets \{T\:|\:T\:\in\:S_t\:\land T$ is not used $\}$}\label{line:check_used}
  \State{$steps \gets \emptyset, ppls \gets \emptyset$}
  \ForEach{$T \in S_t$}
  \State{$steps \gets steps \cup predict(T,\:Groupby)$}
  \EndFor\label{line:loop_groupby}
  \ForEach{$T_1, T_2 \in S_t$}
  \State{$steps \gets steps \cup predict(T_1,\:T_2,\: Join)$}
  \State{$steps \gets steps \cup predict(T_1,\:T_2,\: Union)$}
  \EndFor
  \ForEach{$s \in steps$}
    \State{$ppls.append(PPL(p.steps + s))$}
  \EndFor
  \State{return $ppls$}
  \EndProcedure
  
  \end{algorithmic}
  \end{algorithm}

\subsection{Diversity Object Search}
\label{subsection:diversity}
As descibed in the Section~\ref{sec:algo_overview}, for each depth during the 
search, we will keep W most promising partial pipelines to continue the 
further search. Algorithm~\ref*{algo:diversity_search} shows how we select
the top W partial pipelines through the diversity object search. We aim to 
maximize the operator joint probability with all columns in $T^{tgt}$ mapped
and the FD/Key constraints discovered from $T^{tgt}$ satisfied. So we divide our 
W search window W by 3, with W/3  selecting the pipelines which 
maps the most columns, W/3  selecting the pipelines which satisfies
the most FD/Key constriants, and W/3  selecting the pipelines which
has the highest joint operator probability.

We will then introducte how to calcuate column correspondence,
FD/Key constraints mapping, and operator joint probability.

\begin{algorithm}[h]
  \caption{Diversity Object Search}
  \label{algo:diversity_search}
{\color{blue}$\#$ Input: pipelines $ppls$, target output $T^{tgt}$, window size W}\\
{\color{blue}$\#$ Output: Top W pipelines}
\begin{algorithmic}[1]
  \Procedure{GetTop}{$ppls, T^{tgt}, W$}
  \State{Top W/3 $Rank(ppls,\:$ `Column Correspondence'$)$ +}
  \State{Top W/3 $Rank(ppls,\:$ `FD/Key Constraints'$)$ +}
  \State{Top W/3 $Rank(ppls,\:$ `Joint Operator Probability'$)$}
  \EndProcedure
  
  \end{algorithmic}
  \end{algorithm}


1. Column Correspondence:

Given two tables, an output table generated from a partial pipeline 
$T^g$ with m columns, and an target output table $T^{tgt}$ with n columns,
 we will generate m * n column pairs. We filter the column pairs by checking  whether 
 they are of the same type. 
 
 For categorical column pairs, we calculate the Jaccard value
 between using the following formular. If the jaccard value of 
 certain pair exceeds the predefined threshold, we consider two 
 columns could be mapped to each other. 

\begin{center}
    $\mathrm{J(A,B)} = |A \cap B| / |A \cup B|$
\end{center}

For numerical column pairs, we we compute the min/max range of $col_1$ and $col_2$,
and calculate the intersection of the ranges over the union of the ranges
as shown in Algorithm~\ref*{algo:range_overlap}. If the range overlap value of 
certain pair exceeds the predefined threshold, we consider two 
columns could be mapped to each other. 

\begin{algorithm}[h]
  \caption{Range Overlap}
  \label{algo:range_overlap}
{\color{blue}$\#$ Input: column 1  $col_1$, column 2 $col_2$}\\
{\color{blue}$\#$ Output: range overlap value} 
\begin{algorithmic}[1]
  \Procedure{GetRangeOverlap}{$ppls, T^{tgt}, W$}
  \State{$l1, r1 \gets range(col_1), l2, r2 \gets range(col_2)$}
  \State{$overlap \gets min(r1, r2) - max(l1, l2)$}
  \State{$overlap \gets 0 $ if overlap < 0}
  \State{$totalRange \gets max(r1, r2) - min(l1, l2)$}
  \State{return $overlap / totalRange$}
  \EndProcedure
\end{algorithmic}
\end{algorithm}

For columns in target output table $T^{tgt}$ which do not have corresponding 
columns in input table after using above two methods, we calculate 
the  average pattern distance to find their mapped columns. 
As described in Algorithm~\ref{algo:average_dis}, we firstly preprocess column pair (A,B) by 
transforming each row into `pattern', which is to use `X' to represent uppercase letter,
`x' to represent lowercase letter, and `d' to represent digital letter. 
For each row in $col_1$, we find the minimum relative edit distance with 
rows in $col_2$, and vice versa. 
The function \texttt{relaDis} (Line~\ref*{line:rela_dis})  is used to calculate the  
relative edit distance of two words through dividing 
the Levenshtein distance between them by the sum of their length. 
All minimum relative distance will be added and diveded by the total length
of these two columns. If the average range distance between two columns
is smaller than the predefined value, we could map them together. 




\begin{algorithm}[h]
  \caption{Average Pattern Distance}
  \label{algo:average_dis}
{\color{blue}$\#$ Input: 2 columns: $col_1$, $col_2$}\\
{\color{blue}$\#$ Output: Average Pattern Distance}
\begin{algorithmic}[1]
  \Procedure{GetAveragePatternDistance}{$ppls, T^{tgt}, W$}
  \State{$col_1 \gets getPattern(col_1), col_2 \gets getPattern(col_2)$}
  \State{$dis \gets 0$}
  \ForEach{$v_1 \in col_1$}
  \State{$dis \gets dis + min(\{relaDis(v_1, v_2) | v_2 \in col_2\})$}\label{line:rela_dis}
  \EndFor
  \ForEach{$v_2 \in col_2$}
  \State{$dis \gets dis + min(\{relaDis(v_2, v_1) | v_1 \in col_1\})$}
  \EndFor
  \State{return $dis / (len(col_1) + len(col_2))$}
  \EndProcedure
\end{algorithmic}
\end{algorithm}
2. FD/Key Constraints
We extend FDTool~\cite{buranosky2018fdtool} to extract FD/Key constraints 
$fds$ and $keys$ from  output table $T^{tgt}$. For each key and fd, we check 
whether they are satisfied through the mapped columns. For example, if $col_1$
in $T^{tgt}$ is a key, and $col_2$ in $T^g$ is mapped to $col_1$, we need to
check whether $col_2$ is a key inside $T^g$. We compute the FD/Key constraints 
cover ratio through dividing the number satisfied FD/Key contraints 
in $T^g$  by the total number of FD/Key contraints in $T^{tgt}$.

3. Joint Operator Probability

The calculation of the joint operator probability is rather intuitive,
we simply multiply the single operator probability $P_\mathbf{T}(O)$ for
every step in the partial pipelines.


\subsection{Last Step Tuning}
In the last step tuning state, given the candidate pipelines whose output
either lack of one FD constraint or one Key constraint, we tune the pipeline
based on the following rules:

1. Missing Key constraints

For a candidate pipeline whose output table $T^g$ satisfies all but one 
Key constraints $key$  in $T^{tgt}$, we will tune the pipeline by adding a GroupBy
step on the columns mapped to $key$ in the end. 


2. Missing FD constraints

For a candidate pipeline whose output table $T^g$ satisfies all but one 
FD constraints in $T^{tgt}$, we will extend the pipeline by adding a GroupBy
step on the columns mapped to $key$ producing output table $T^{groupby}$, followed 
by a  Join Step with $T^g$, $T^{groupby}$ as input and $key$ as join columns.

\subsection{String Transformation}


==> experiment__Yeye_He_s_conflicted_copy_2021-03-01_.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Experiments}
\label{sec:experiments}
We evaluate different pipeline synthesis algorithms
by both success rates and efficiency.
All experiments were performed on a Linux VM from a
commercial cloud, with 16 virtual CPU
and 64 GB memory. Variants of \sj{}  
are implemented in Python 3.6.9. 

We make our software artifacts and scripts available,
so that experiment results reported here can be reproduced\footnote{\small Please follow the README file to reproduce results: \url{https://www.dropbox.com/sh/574gox2waefn5cj/AADxltcc8K_ffFEDew0UPTIDa?dl=0}}.

\subsection{Evaluation Datasets}
We created two benchmarks of data pipelines to evaluate the
task of pipeline synthesis, which will be released
on GitHub to facilitate future research.


\textbf{The GitHub Benchmark.}
Our first benchmark, referred to as \textsf{GitHub}, 
consists of real data pipelines 
authored by developers and data scientists, which we
harvested at scale from GitHub. Specifically, we crawled
Jupyter notebooks from GitHub, and
replayed them programmatically on corresponding data sets
(from GitHub, Kaggle, and other sources) to reconstruct the
pipelines authored by experts, in a manner similar
to~\cite{auto-suggest}. 
We filter out pipelines 
that are likely duplicates (e.g., copied/forked from other pipelines), 
and ones that are trivially small (e.g., input tables have 
less than 10 rows). These human-authored
pipelines become our ground-truth for by-target synthesis.

We group these pipelines based on \textit{pipeline-lengths}, 
defined as the number of steps in a pipeline. Longer pipelines are intuitively
more difficult to synthesize, because the space of possible
pipelines grows exponentially with pipeline-lengths.
We randomly sample
100 pipelines of length 
\{1, 2, 3, 4, 5, [6-8], 9+\}, for a total of 700 pipelines, as our benchmark.



%For each length group described in Table~\ref{tab:github-bench}, we randomly 
%selected 100 of them as the test pipelines. We also randomly sampled 1000 
%pipelines used as the training data for our learning-based synthesis.

%\begin{table}[h]
%    \centering
%    \caption{Pipelines from Github groupby Length}
%    \resizebox{0.7\columnwidth}{!}{
%    \begin{tabular}{lrrrrrrr}
%        \toprule
%        length & 1 & 2 & 3 & 4 & 5 & 6-8 & \textgreater 9 \\
%        \bottomrule
%    \end{tabular}
%    }
%    \label{tab:github-bench}  
%\end{table}

\textbf{The Commercial Benchmark.}
Since there are a large number of commercial systems that also 
help users build complex data pipelines 
(e.g., vendors discussed
in Section~\ref{sec:intro}),
we also create a second benchmark referred to as \textsf{Commercial}
using pipelines from these commercial vendors.
 We sample 4 leading
vendors~\footnote{\small Alteryx~\cite{alteryx}, SQL Server Integration Services~\cite{ssis},
Microsoft Power Query~\cite{powerbi},
Microsoft Azure Data Factory~\cite{adf}}, and manually
collect 16 demo pipelines from official tutorials of
these vendors, as ground-truth pipelines for synthesis.

Recall that these commercial tools help less-technical users build pipelines
step-by-step (e.g., via drag-and-drop) -- with this benchmark
we aim to understand what fraction of these pipelines 
(for canonical ETL and data-prep use cases) 
can be automated using \sj. 

Note that for learning-based
\sj, we use models trained on the \textsf{GitHub} pipelines
to synthesize pipelines in  \textsf{Commercial},
which is a clear test of generalizability of learned synthesis algorithms.


\begin{table}
\centering
    \caption{Characteristics of pipeline synthesis benchmarks.}
	 \label{tab:benchmarks}
\begin{scriptsize}
\begin{tabular}{lrrrr}
    \toprule
       Benchmark & \# of pipelines & \begin{tabular}{@{}c@{}}avg. \# of \\ input files \end{tabular}    & \begin{tabular}{@{}c@{}}avg. \# of \\ input cols \end{tabular} & \begin{tabular}{@{}c@{}}avg. \# of \\ input rows \end{tabular}  \\
        \midrule
        \textsf{GitHub}  & 700     & 6.6 & 9.1 &   4274     \\
        \midrule
        \textsf{Commercial}   & 16     & 3.75 & 8.7 & 988     \\
    \bottomrule     
    \end{tabular}
\end{scriptsize}
\end{table}

\begin{comment}
\begin{table}[h]
\centering
\caption{Pipelines for \textsf{Commercial}}
\begin{tabular}{rrrrrr}
    \toprule
    Software & Alteryx & PQ & SSIS & ADF & Sum\\
    \midrule
    Number & 8 & 1 & 3 & 3 & 16\\
    \bottomrule
\end{tabular}  
\label{tab:commerce-bench}  
\end{table}
\end{comment}

\subsection{Methods Compared}
Because ``by-target'' is a new paradigm 
not studied in the literature before,
we compare \sj{} with 
methods mostly from the ``by-example'' literature.
%(which require users to provide a complete output table
%matching the given input tables and is pretty difficult in practice).


$\bullet$ \textbf{SQL-by-example}~\cite{sql-by-example}. This
recent ``by-example'' approach synthesizes SQL queries
using a matching pair of input/output table.  Like other
``by-example'' approaches, because \textsf{SQL-by-example} 
requires a precise output-table matching
the given input, the fuzzy
``target-schema'' used by \sj{} is insufficient. In order to 
make it work, we provide the exact output from 
the ground-truth pipelines to \textsf{SQL-by-example}.
We use the author's 
implementation~\cite{sql-by-example-github}, and set a timeout
of 3600 seconds per task. {\color{blue} JW: we also down sampled the input 
to 5 rows considering the time limit}




$\bullet$ \textbf{SQL-by-example-UB}~\cite{sql-by-example}. 
Because \textsf{SQL-by-example} frequently
times-out on large input tables, we analyze its
theoretical upper-bound of ``coverage'', based on the operators
it supports in its DSL (Join, Aggregation, Union, etc.). 
If all operators used in a benchmark pipeline are included 
in its DSL, we mark the pipeline as ``covered'' in this upper-bound
analysis (these pipelines can in theory be covered with 
a sufficiently large amount of time to search).


$\bullet$ \textbf{Query-by-output-UB (QBO-UB)}~\cite{qbo}.
\textsf{Query-by-output} is another influential ``by-example'' approach that
synthesize SQL pipelines based on input/output tables.
Since its code is not publicly available, we also evaluate its 
theoretical upper-bound coverage based on the operators
in its DSL, like in \textsf{SQL-by-example-UB} above.

\begin{comment}
$\bullet$ \textbf{Auto-Pandas}~\cite{bavishi2019autopandas}.
\textsf{Auto-Pandas} is another ``by-example'' approach that
synthesize Pandas programs instead of SQL statements,
by learning from synthetically-generated programs. 
We use the authors' implementation~\cite{Auto-Pandas-code}
in our experiments, and like in \textsf{SQL-by-Example} we
feed \textsf{Auto-Pandas} with ground-truth output-tables
matching the given input tables, in order to make it function
properly.  \todo{}
\end{comment}


$\bullet$ \textbf{Auto-Suggest}~\cite{auto-suggest}.
Auto-Suggest is a recent approach that
automates \textit{single} table-manipulation steps (e.g., Join, 
Pivot, GroupBy) by learning from Jupyter Notebooks
on GitHub. We use \textsf{Auto-Suggest} to synthesize
multi-step pipelines, by greedily finding top-K most
likely steps at each intermediate pipeline stage.





$\bullet$ \textbf{\sj}. This is our proposed method.
We report results from three variants, namely the search-based 
\sjs, the supervised-learning-based \sjsl, 
and the reinforcement-learning-based \sjrl.

For learning-based methods,
we randomly sample 1000 pipelines with at least 2 steps
as training data that are completely disjoint
with the test pipelines -- specifically, we 
not only make sure that the train/test pipelines have no overlap, 
but also the data files used by the train/test pipelines have
no overlap (e.g., if a pipeline
using ``titanic.csv'' as input is selected in the test set, no pipelines
using the same input-file would be selected into training ). {\color{blue} JW: the filtering is based on the column names and input shape 
instead of the name of the input files, no pipelines
using the input-file which have the same column names and shape with `titanic.csv' would be selected into training} This ensures
that test pipelines are completely new to learning-based 
synthesizers, which can better test generalization of the synthesis algorithms.
Because learning-based variants produce
randomized results, we report numbers 
averaged over 5 runs.



\subsection{Evaluation Method and Metric}
\textbf{Accuracy.} Given a benchmark of $P$ pipelines,
accuracy measures the fraction of pipelines that can
be successfully synthesized, or $\frac{\text{num-succ-synthesized}}{P}$.
%\todo{top K = 12} 

\textbf{Mean Reciprocal Rank (MRR).} 
MRR is a standard metric that measures the quality 
of ranking~\cite{ir}.  In our setting of pipeline synthesis, 
a synthesis algorithm returns a ranked list of $K$ candidate pipelines
for each test case,
ideally with the correct pipeline ranked high (at top-1). 
The \textit{reciprocal-rank}~\cite{ir} in this case is defined as 
$ \frac{1}{rank}$, where $rank$ is the rank-position of the first 
correct pipeline in the candidates 
(if no correct pipeline exists in top-K then the 
reciprocal-rank is 0). For a benchmark with $P$ test pipelines, 
the \textit{Mean Reciprocal Rank} is the mean 
reciprocal ranks over all pipelines, defined as: 

\begin{center}
    $\mathrm{MRR} = \frac 1 P \sum_{i=1}^{P} \frac 1 {rank_i}$
\end{center}

We note that MRR is in the range of [0, 1], with 1 being perfect
(all correct pipelines ranked at top-1).

%\textbf{Latency.} 

\subsection{Comparison of Synthesis}

\textbf{Overall comparisons.} Table~\ref{tab:overall-github}
and Table~\ref{tab:overall-commercial} show an overall comparison
on the \textsf{GitHub} and
\textsf{Commercial} benchmark, respectively, measured
using accuracy, MRR, and latency. We report average
latency on successfully-synthesized
cases, because some baselines fail to synthesize and would 
only timeout after hours of search.

As can be seen from
the tables, \sj{} based methods 
can consistently synthesize 60-70\% of pipelines
within 10-20 seconds across the two benchmarks,
which is substantially more efficient and effective than
alternative methods.  

While our search-based 
\sjs{} is already effective, the RL-based 
\sjrl{} is slightly better in terms of accuracy.
The advantage of \sjrl{} over \sjs{} is more
pronounced in terms of MRR, which is somewhat expected
because learning-based methods are
likely more effective in fine-grained ranking decisions 
than a more coarse-grained optimization objective
used in our search-based variant (Equation~\eqref{eqn:obj}).

We note that because our input/output tables are from
real pipeline and are typically large 
(as shown in Table~\ref{tab:benchmarks}),
existing by-example synthesis methods like
\textsf{SQL-by-Example} frequently timeout 
after hours of search, because their search methods are
exhaustive in nature, which fail to
leverage key properties like FD and Key constraints
to prioritize search. We should also note that
even theoretical upper-bounds of existing by-example methods
(based on their DSL) are substantially smaller than 
\sj, showing the richness of the operators supported in our methods.

\begin{table*}
\vspace{-10mm}
\parbox{.45\linewidth}{
\centering
    \caption{Results on the \textsf{GitHub} benchmark}
	 \label{tab:overall-github}
\begin{scriptsize}
\begin{tabular}{lrrr}
    \toprule
        & Accuracy & MRR  & Latency (seconds) \\
        \midrule
        \sjs   & 76.6\%     & 0.724 & 18       \\
        \midrule
        \sjsl  & 73.7\%     & 0.583 & 20     \\
        \midrule
        \sjrl  & \textbf{76.9\%}     & \textbf{0.738} & 21       \\ \hline
        \midrule
        SQL-by-Example & 14.7\%     & 0.147 & 49 \\
        \midrule
        SQL-by-Example-UB & 56\%    & 0.56 & - \\
        \midrule
        Query-by-Output-UB & 15.7\%    & 0.157 & - \\
        \midrule
        Auto-Suggest & 29.7\%   & 0.297 & 11 \\
    \bottomrule     
    \end{tabular}
\end{scriptsize}
}
\hfill
\parbox{.45\linewidth}{
\centering
    \caption{Results on the \textsf{Commercial} benchmark}
	 \label{tab:overall-commercial}
\begin{scriptsize}
 \begin{tabular}{lrrr}
    \toprule
        & Accuracy & MRR  & Latency (seconds) \\
        \midrule
        \sjs   & 62.5\%     & 0.593 & 13       \\
        \midrule
        \sjsl   & \textbf{68.8\%}     & 0.583 & 14     \\
        \midrule
        \sjrl  & \textbf{68.8\%}     & \textbf{0.645} & 14       \\ \hline
        \midrule
        SQL-by-Example & 19\%     & 0.15 & 64 \\
        \midrule
        SQL-by-Example-UB & 37.5\%    & 0.375 & - \\
        \midrule
        Query-by-Output-UB & 18.8\%    & 0.188 & - \\
        \midrule
        Auto-Suggest & 25\%   & 25 & 13 \\
    \bottomrule     
    \end{tabular}
\end{scriptsize}
}
\end{table*}




\begin{figure*}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/accuracy-comp.pdf}
    \caption{Accuracy results by pipeline-lengths on the \textsf{GitHub} benchmark.}
    \label{fig:acc-comp}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/mrr-comp.pdf}
    \caption{MRR results by pipeline-lengths on the \textsf{GitHub} benchmark.}
    \label{fig:mrr-comp}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/latency-comp.pdf}
    \caption{Latency results by pipeline-lengths on the \textsf{GitHub} benchmark}
    \label{fig:latency-comp}
\endminipage
\end{figure*}


\textbf{Synthesis Quality.}
Figure~\ref{fig:acc-comp} and Figure~\ref{fig:mrr-comp} 
show detailed comparisons of 
accuracy and MRR, between different 
methods on the \textsf{GitHub} benchmark.
Test pipelines are bucketized into 7 groups based on their
lengths (shown as the x-axis), with longer pipelines being
more difficult to synthesize. It can be seen
that \sjrl{} and \sjs{} are comparable in terms of quality,
with \sjrl{} being slightly better in terms of MRR. We can see
that \sjrl{} is noticeably better than \sjsl{}, showing the benefit of
using RL to proactively select
examples to learn from.  

All \sj{} variants are substantially better 
than \textsf{QBO} and \textsf{SQL-by-example} baselines. 
We note that \textsf{SQL-by-example} fails to synthesize
any pipeline longer than 3-steps within our 1 hour timeout limit, 
showing its limited efficacy when dealing with 
large input tables from real pipelines.

\textbf{Latency.}
Figure~\ref{fig:latency-comp} shows a comparison of the
average latency to successfully synthesize a pipeline between all methods
on the \textsf{GitHub} benchmark, bucketized by
pipeline-lengths (x-axis). While all \sj{} methods have
comparable latency, \textsf{SQL-by-example} 
requires 20x-7x more time to synthesize pipelines up to 3 steps
(it times-out on longer pipelines).


\textbf{Pipeline simplification.} As discussed earlier, 
the pipelines we synthesize can be simpler (with fewer
number of steps) than pipelines
authored by humans, but still being
semantically equivalent. Figure~\ref{fig:ppl-sim}
shows a real example from GitHub, where 
the human-written pipeline would 
group-by on column \texttt{Sex} for four times with 
different aggregation (\texttt{mean}, 
\texttt{count}, \texttt{median}, \texttt{max}),
before joining them back on the column \texttt{Sex}. 
A synthesized pipeline from \sj{} is a one-liner in this
case, which is much more succinct. While this example
is intuitive, there are many more involved examples of
simplifications, such as a join between K similar files 
followed by one unpivot, is equivalent
to one unpivot on each of the K file followed by (K-1) union, etc.

Out of the 700 pipeline in the
\textsf{GitHub} benchmark, our synthesized pipelines are
simpler (with less number of steps) on 90 cases (12.85\%).
Pipeline simplification is an interesting use case and
an added benefit of \sj. %and even ``semantic translation''
%from one language to another (e.g., from SQL to Pandas).

    \begin{figure}[h]
        \centering
        \subfigure[Human-authored pipeline]{ 
            \includegraphics[width=\columnwidth]{figures/ppl_l7.pdf}
            \label{fig:beforeSim}
            }
        \subfigure[A synthesized pipeline with a smaller number of steps]{ 
            \includegraphics[width=\columnwidth]{figures/p7_simplified.png}
            \label{fig:afterSim}
            }
        % \includegraphics[width=\columnwidth]{figures/ppl_l7.pdf}
        \caption{An example pipeline simplified after synthesis.}
    % to be replaced by real results
        \label{fig:ppl-sim}
    \end{figure}




\subsection{Sensitivity Analysis}

\begin{figure*}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/latency-t-crop.pdf}
    \caption{Latency by search width $K$.}
    \label{fig:latency-window}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/acc-trend.pdf}
    \caption{Quality by search width $K$.}
    \label{fig:acc-window}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/topk-trend.pdf}
    \caption{Accuracy/MRR by varying parameter choices M (on length-4 pipelines).}
    \label{fig:topk}
\endminipage
\end{figure*}

\textbf{Varying Search Width $K$.} As discussed in
Section~\ref{sec:algo}, \sj{} uses a form of beam search by
keeping top-$K$ most promising partial pipelines 
in \textsf{GetPromisingTopK()} and \textsf{GetFinalTopK()}
of Algorithm~\ref{algo:meta} to reduce the search space.
We perform a sensitivity analysis to study the effect of varying $K$
on synthesis quality and latency, which are
shown in Figure~\ref{fig:latency-window}
and Figure~\ref{fig:acc-window}, respectively. 
We vary $K$ from 3 to 24 using a step size of 3, which
is shown as the x-axis in the figures.

Figure~\ref{fig:latency-window} shows that 
the overall latency increases roughly linearly with 
$K$, which is expected. It is encouraging to see
that the slope of increase is not significant.

Figure~\ref{fig:acc-window} shows the accuracy with a larger $K$.
We can see that the accuracy plateaus quickly after $K$ reaches 12,
suggesting that our algorithm is effective in picking out 
promising partial candidates without needing to keep an excessively
large window of candidates.




\textbf{Varying single-operator top-M parameter choices.}
Recall that in \textsf{AddOneStep()}
of Algorithm~\ref{algo:meta}, 
we consider top-$M$ parameter choices for each 
possible operator when extending partial pipelines.
 We evaluate in Figure~\ref{fig:topk}
the effect of varying $M$ (from 1 to 8) on result quality.
It can be seen that we get better
accuracy from $M=1$ to $M=2$ 
(because sometimes the desired parameter choice is
ranked at top-2),
but slightly worse MRR (because ranking becomes more difficult
with more candidates). We observe no accuracy or MRR improvement
beyond $M=2$, suggesting that the single-operator 
top-M (\cite{auto-suggest}) is fairly reliable with the 
correct choice ranked among the top-2 in most cases.

%we run the search-based alogrithm on pipelines of length 4 with different top k  paramters range from 1 to 8. 

\textbf{Varying input table sizes.}
We sample 10 pipelines from the \textsf{GitHub} benchmark
with input tables that have over 100k rows. 
We down-sample their largest input table to 
100k, 10k, 1k, and 100 rows, respectively, and
execute our synthesis algorithms in order 
to understand how input table sizes
influence synthesizing latency. 

Figure~\ref{fig:table-size} shows that the latency of
our synthesis increases relatively slowly compared to input row --
as the input size increases by 1000x, our latency increases by 3x, 
suggesting that our synthesis has good scalability on real 
data pipelines tasks (which likely have large tables).



\begin{figure*}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/size-trend.pdf}
    \caption{Latency by input table sizes on same pipeline tasks.}
    \label{fig:table-size}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/data-size-l5.pdf}
    \caption{Accuracy results by training iterations (on length-5 pipelines)}
	\label{fig:acc-iteration}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/data-size-l5-mrr.pdf}
    \caption{MRR  results by training iterations (on length-5 pipelines)}
	\label{fig:mrr-iteration}
\endminipage
\end{figure*}



\textbf{Varying the number of training iterations.}
For learning-based methods \sj, we 
report in Figure~\ref{fig:acc-iteration} and Figure~\ref{fig:mrr-iteration}
the accuracy/MRR with different numbers of training iterations. 
As can be seen,
both results become fairly stable after
10 iterations. The average execution time 
is about 28 minutes for each iteration.




\subsection{Ablation Studies}
In order to understand the importance of key components
in \sj, we perform an ablation study shown 
in Figure~\ref{fig:ablation-accuracy}.

\textbf{Without FD/Key constraints.}
Recall that FD/Key constraints inferred from output-schema
are key properties we leverage in \sj{} that drastically
reduce the search space for synthesis, which were
not previously exploited in the literature. 
The yellow bars in Figure~\ref{fig:ablation-accuracy}
show that without  these constraints, 
the accuracy results drop consistently for pipelines of
different lengths.



\begin{figure}
\minipage{0.23\textwidth}
  \includegraphics[width=\linewidth]{figures/ablation-acc.pdf}
    \caption{Ablation studies for accuracy.}
	\label{fig:ablation-accuracy}
\endminipage\hfill
\minipage{0.23\textwidth}
  \includegraphics[width=\linewidth]{figures/error-analysis.pdf}
    \caption{Error Analysis.}
	\label{fig:error-analysis}
\endminipage
\end{figure}





\textbf{Without column-mapping}.
When column-mapping between input/output columns are
no longer leveraged, it is not only infeasible to estimate 
``progress'' in terms of column coverage, but not impossible 
to leverage FD/key constraints where column-mapping is a prerequisite.
As can be seen, the green bars show a more significant drop in quality.

\textbf{Without single-operator probabilities.}
Finally, when the top-K choices from single-operator models
are used but their probability scores are removed,
the red bars suggest a more modest drop in accuracy.
This indicates that the FD/key constraints serve as
important constraints to greatly reduce the feasible solutions,
making the ranking of candidates from single-operator probabilities
less critical.

%\todo{Ablation, (optional) without using attribute-names in schema-matching?}

\subsection{Error Analysis}
In this section, we present the error analysis on the pipelines 
Auto-Pipeline failed to synthesize correctly. As shown in 
Figure~\ref{fig:error-pipeline}, the 2-step pipeline firstly conducts a 
GroupBy on `Sex' to compute the average `Fare`, and then conducts a 
Join back on `Sex' with the original input. And then it drops the
`Sex' column in the output schema. The final `drop column' operation makes
Auto-Pipeline unable to find the FD constraint thus considering the 
input table already meets all the requriement to be a candidate pipeline. 

To understand how FD/key will affect the synthesis, we categorize the successful
and failed pipelines by whether the target schema has both FD/key, only Fd, only key,
and no FD or key. As shown in Figure~\ref{fig:error-analysis}, the failure rate
of pipelines with no FD or key is highest, which indicates that FD/key constraints
to be a very important specification in our synthesis. 

\todo{also add the error analysis example on the slide deck here}.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figures/error-pipeline.png}
  \caption{Example of failed pipeline}
  \label{fig:error-pipeline}
\end{figure}


==> experiment__Yeye_He_s_conflicted_copy_2021-03-01_1_.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Experiments}
\label{sec:experiments}
We evaluate different pipeline synthesis algorithms
by both success rates and efficiency.
All experiments were performed on a Linux VM from a
commercial cloud, with 16 virtual CPU
and 64 GB memory. Variants of \sj{}  
are implemented in Python 3.6.9. 

We make our software artifacts and scripts available,
so that experiment results reported here can be reproduced\footnote{\small Please follow the README file to reproduce results: \url{https://www.dropbox.com/sh/574gox2waefn5cj/AADxltcc8K_ffFEDew0UPTIDa?dl=0}}.

\subsection{Evaluation Datasets}
We created two benchmarks of data pipelines to evaluate the
task of pipeline synthesis, which will be released
on GitHub to facilitate future research.


\textbf{The GitHub Benchmark.}
Our first benchmark, referred to as \textsf{GitHub}, 
consists of real data pipelines 
authored by developers and data scientists, which we
harvested at scale from GitHub. Specifically, we crawled
Jupyter notebooks from GitHub, and
replayed them programmatically on corresponding data sets
(from GitHub, Kaggle, and other sources) to reconstruct the
pipelines authored by experts, in a manner similar
to~\cite{auto-suggest}. 
We filter out pipelines 
that are likely duplicates (e.g., copied/forked from other pipelines), 
and ones that are trivially small (e.g., input tables have 
less than 10 rows). These human-authored
pipelines become our ground-truth for by-target synthesis.

We group these pipelines based on \textit{pipeline-lengths}, 
defined as the number of steps in a pipeline. Longer pipelines are intuitively
more difficult to synthesize, because the space of possible
pipelines grow exponentially with the pipeline-length.
  For our synthesis benchmark, we randomly sample
100 pipelines of length 
\{1, 2, 3, 4, 5, [6-8], 9+\}, for a total of 700 pipelines,
to test all synthesis algorithms.



%For each length group described in Table~\ref{tab:github-bench}, we randomly 
%selected 100 of them as the test pipelines. We also randomly sampled 1000 
%pipelines used as the training data for our learning-based synthesis.

%\begin{table}[h]
%    \centering
%    \caption{Pipelines from Github groupby Length}
%    \resizebox{0.7\columnwidth}{!}{
%    \begin{tabular}{lrrrrrrr}
%        \toprule
%        length & 1 & 2 & 3 & 4 & 5 & 6-8 & \textgreater 9 \\
%        \bottomrule
%    \end{tabular}
%    }
%    \label{tab:github-bench}  
%\end{table}

\textbf{The Commercial Benchmark.}
Since there are a large number of commercial systems that also 
help users build complex data pipelines 
(e.g., vendors discussed
in Section~\ref{sec:intro}),
we create a second benchmark referred to as \textsf{Commercial},
using pipelines from commercial vendors.
 We sample 4 leading
vendors~\footnote{Alteryx~\cite{alteryx}, SQL Server Integration Services~\cite{ssis},
Microsoft Power Query~\cite{powerbi},
Microsoft Azure Data Factory~\cite{adf}}, and manually
collect 16 demo pipelines from official tutorials of
these vendors, as pipelines for synthesis.

Recall that these commercial tools help users build pipelines
step-by-step (via drag-and-drop) -- with this benchmark
we aim to understand what fraction of pipelines from standard
commercial use cases (ETL and data-prep) 
can be automated using our proposed \sj. 

Note that for learning-based
\sj, we use models trained on the \textsf{GitHub} pipelines
to synthesize pipelines from the  \textsf{Commercial} benchmark,
which also tests the generalizability of the synthesis algorithms.


\begin{table}
\centering
    \caption{Characteristics of pipeline synthesis benchmarks.}
	 \label{tab:benchmarks}
\begin{scriptsize}
\begin{tabular}{lrrrr}
    \toprule
       Benchmark & \# of pipelines & \begin{tabular}{@{}c@{}}avg. \# of \\ input files \end{tabular}    & \begin{tabular}{@{}c@{}}avg. \# of \\ input cols \end{tabular} & \begin{tabular}{@{}c@{}}avg. \# of \\ input rows \end{tabular}  \\
        \midrule
        \textsf{GitHub}  & 700     & 6.6 & 9.1 &   4274     \\
        \midrule
        \textsf{Commercial}   & 16     & 3.75 & 8.7 & 988     \\
    \bottomrule     
    \end{tabular}
\end{scriptsize}
\end{table}

\begin{comment}
\begin{table}[h]
\centering
\caption{Pipelines for \textsf{Commercial}}
\begin{tabular}{rrrrrr}
    \toprule
    Software & Alteryx & PQ & SSIS & ADF & Sum\\
    \midrule
    Number & 8 & 1 & 3 & 3 & 16\\
    \bottomrule
\end{tabular}  
\label{tab:commerce-bench}  
\end{table}
\end{comment}

\subsection{Methods Compared}
Because ``by-target'' is a new paradigm 
not studied in the literature before,
we compare \sj{} with 
methods mostly from the ``by-example'' literature.
%(which require users to provide a complete output table
%matching the given input tables and is pretty difficult in practice).


$\bullet$ \textbf{SQL-by-example}~\cite{sql-by-example}. This is a
recent ``by-example'' approach that synthesizes SQL queries
based on input/output tables.  Like other
``by-example'' approaches, because \textsf{SQL-by-example} 
requires users to provide a precise output-table matching
the given input-tables, the fuzzy and inexact
``target-schema'' used by \sj{} is insufficient. In order to 
make it work, we provide the exact output from 
the ground-truth pipelines to \textsf{SQL-by-example}.
We use the author's 
implementation~\cite{sql-by-example-github}, and set a timeout
of 3600 seconds per task. For cases where this method fails
due to timeout we give it another try using small input tables with
5 sampled rows only.




$\bullet$ \textbf{SQL-by-example-UB}~\cite{sql-by-example}. 
Because \textsf{SQL-by-example} frequently
times-out on large input tables, we analyze its
theoretical upper-bound of ``coverage'', based on the operators
it supports in its DSL (Join, Aggregation, Union, etc.). 
If all operators used in a benchmark pipeline are included 
in its DSL, we mark the pipeline as ``covered'' in this 
theoretical upper-bound analysis.


$\bullet$ \textbf{Query-by-output-UB (QBO-UB)}~\cite{qbo}.
\textsf{Query-by-output} is another influential ``by-example'' approach that
synthesizes SQL pipelines by input/output tables.
Since its code is not publicly available, we also evaluate its 
theoretical upper-bound coverage based on its operators.

\begin{comment}
$\bullet$ \textbf{Auto-Pandas}~\cite{bavishi2019autopandas}.
\textsf{Auto-Pandas} is another ``by-example'' approach that
synthesize Pandas programs instead of SQL statements,
by learning from synthetically-generated programs. 
We use the authors' implementation~\cite{Auto-Pandas-code}
in our experiments, and like in \textsf{SQL-by-Example} we
feed \textsf{Auto-Pandas} with ground-truth output-tables
matching the given input tables, in order to make it function
properly.  \todo{}
\end{comment}


$\bullet$ \textbf{Auto-Suggest}~\cite{auto-suggest}.
Auto-Suggest is a recent approach that
automates \textit{single} table-manipulation steps (e.g., Join, 
Pivot, GroupBy) by learning from Jupyter Notebooks
on GitHub. We use \textsf{Auto-Suggest} to synthesize
multi-step pipelines, by greedily finding top-K most
likely operators at each step.





$\bullet$ \textbf{\sj}. This is our method, and we 
report results from three variants: 
\sjs, \sjrl, and \sjsl (using supervised learning),
which differ in how \textsf{GetPromisingTopK()} is instantiated.

For learning-based methods,
we randomly sample 1000 pipelines with at least 2 steps
as training data that are completely disjoint
with the test pipelines -- specifically, we 
not only make sure that the train/test pipelines have no overlap, 
but also the data files used by the train/test pipelines have
no overlap (e.g., if a pipeline
using ``titanic.csv'' as input is selected in the test set, no pipelines
using an input-file with the same schema would be selected into training). 
This ensures that test pipelines are completely unseen to learning-based 
synthesizers. Because learning-based variants produce
randomized results, we report numbers 
averaged over 5 runs.



\subsection{Evaluation Method and Metric}
\textbf{Accuracy.} Given a benchmark of $P$ pipelines,
accuracy measures the fraction of pipelines that can
be successfully synthesized, or $\frac{\text{num-succ-synthesized}}{P}$.
%\todo{top K = 12} 

\textbf{Mean Reciprocal Rank (MRR).} 
MRR is a standard metric that measures the quality 
of ranking~\cite{ir}.  In our setting,
a synthesis algorithm returns a ranked list of $K$ candidate pipelines
for each test case,
ideally with the correct pipeline ranked high (at top-1). 
The \textit{reciprocal-rank}~\cite{ir} in this case is defined as 
$ \frac{1}{rank}$, where $rank$ is the rank-position of the first 
correct pipeline in the candidates 
(if no correct pipeline is found then the 
reciprocal-rank is 0). For a benchmark with $P$ test pipelines, 
the \textit{Mean Reciprocal Rank} is the mean 
reciprocal rank over all pipelines, defined as: 
\begin{center}
    $\mathrm{MRR} = \frac 1 P \sum_{i=1}^{P} \frac 1 {rank_i}$
\end{center}
We note that MRR is in the range of [0, 1], with 1 being perfect
(all desired pipelines ranked at top-1).

%\textbf{Latency.} 

\subsection{Comparison of Synthesis}

\textbf{Overall comparisons.} Table~\ref{tab:overall-github}
and Table~\ref{tab:overall-commercial} show an overall comparison
on the \textsf{GitHub} and
\textsf{Commercial} benchmark, respectively, measured
using accuracy, MRR, and latency. We report average
latency on successfully-synthesized
cases only, because some baselines would fail to synthesize 
after hours of search.

As can be seen from
the tables, \sj{} based methods 
can consistently synthesize 60-70\% of pipelines
within 10-20 seconds across the two benchmarks,
which is substantially more efficient and effective than
other methods.  

While our search-based 
\sjs{} is already effective, 
\sjrl{} is slightly better in terms of accuracy.
The advantage of \sjrl{} over \sjs{} is more
pronounced in terms of MRR, which is expected
as learning-based methods are better at
understanding the nuance in fine-grained ranking decisions 
than a coarse-grained optimization objective
in our search-based variant (Equation~\eqref{eqn:obj}).

We note that because our input/output tables are from
real pipeline and are typically large 
(as shown in Table~\ref{tab:benchmarks}),
existing by-example synthesis methods like
\textsf{SQL-by-Example} frequently timeout 
after hours of search, because their search methods are
exhaustive in nature. We should also note that
even the theoretical upper-bound coverage of existing by-example methods
(based on their DSL) are substantially smaller than 
\sj, showing the richness of the operators supported in our methods.

\begin{table*}
\vspace{-10mm}
\parbox{.45\linewidth}{
\centering
    \caption{Results on the \textsf{GitHub} benchmark}
	 \label{tab:overall-github}
\begin{scriptsize}
\begin{tabular}{lrrr}
    \toprule
        & Accuracy & MRR  & Latency (seconds) \\
        \midrule
        \sjs   & 76.6\%     & 0.724 & 18       \\
        \midrule
        \sjsl  & 73.7\%     & 0.583 & 20     \\
        \midrule
        \sjrl  & \textbf{76.9\%}     & \textbf{0.738} & 21       \\ \hline
        \midrule
        SQL-by-Example & 14.7\%     & 0.147 & 49 \\
        \midrule
        SQL-by-Example-UB & 56\%    & 0.56 & - \\
        \midrule
        Query-by-Output-UB & 15.7\%    & 0.157 & - \\
        \midrule
        Auto-Suggest & 29.7\%   & 0.297 & 11 \\
    \bottomrule     
    \end{tabular}
\end{scriptsize}
}
\hfill
\parbox{.45\linewidth}{
\centering
    \caption{Results on the \textsf{Commercial} benchmark}
	 \label{tab:overall-commercial}
\begin{scriptsize}
 \begin{tabular}{lrrr}
    \toprule
        & Accuracy & MRR  & Latency (seconds) \\
        \midrule
        \sjs   & 62.5\%     & 0.593 & 13       \\
        \midrule
        \sjsl   & \textbf{68.8\%}     & 0.583 & 14     \\
        \midrule
        \sjrl  & \textbf{68.8\%}     & \textbf{0.645} & 14       \\ \hline
        \midrule
        SQL-by-Example & 19\%     & 0.15 & 64 \\
        \midrule
        SQL-by-Example-UB & 37.5\%    & 0.375 & - \\
        \midrule
        Query-by-Output-UB & 18.8\%    & 0.188 & - \\
        \midrule
        Auto-Suggest & 25\%   & 25 & 13 \\
    \bottomrule     
    \end{tabular}
\end{scriptsize}
}
\end{table*}

\begin{comment}
\begin{table}[]
  \caption{Results on the \textsf{GitHub}/\textsf{Commercial} benchmark}
  \resizebox*{\linewidth}{!}{
    % {\footnotesize Com represents result on Commercial benchmark}
  
  \begin{tabular}{lrrrrrr}
    \toprule
    & \multicolumn{2}{c}{Accuracy}                                        & \multicolumn{2}{c}{MRR}                                           & \multicolumn{2}{c}{Latency (seconds)} \\
    \midrule
    & Github                           & Commercial                     & Github                          & Commercial                      & Github          & Commercial          \\
    \midrule
    \sjs  & 76.6\%                           & 62.5\%                           & 0.724                           & 0.593                           & 18              & 13                  \\
    \midrule
    \sjsl & 73.7\%                           & \textbf{68.8\%} & 0.583                           & 0.583                           & 20              & 14                  \\
    \midrule
    \sjrl & \textbf{76.9\%} & \textbf{68.8\%} & \textbf{0.738} & \textbf{0.645} & 21              & 14                  \\
    \midrule
    \midrule
    SQL-by-Example       & 14.7\%                           & 19\%                             & 0.147                           & 0.15                            & 49              & 64                  \\
    \midrule
    SQL-by-Example-UB    & 56\%                             & 37.5\%                           & 0.56                            & 0.375                           & -               & -                   \\
    \midrule
    Query-by-Output-UB   & 15.7\%                           & 18.8\%                           & 0.157                           & 0.188                           & -               & -                   \\
    \midrule
    Auto-Suggest         & 29.7\%                           & 25\%                             & 0.297                           & 25                              & 11              & 13              \\   
    \bottomrule
  \end{tabular}
  \label{tab:my-table}
  \\
  %{\footnotesize \\Com represents result on Commercial benchmark}
}

  \end{table}
\end{comment}



\begin{figure*}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/accuracy-comp.pdf}
    \caption{Accuracy results by pipeline-lengths on the \textsf{GitHub} benchmark.}
    \label{fig:acc-comp}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/mrr-comp.pdf}
    \caption{MRR results by pipeline-lengths on the \textsf{GitHub} benchmark.}
    \label{fig:mrr-comp}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/latency-comp.pdf}
    \caption{Latency results by pipeline-lengths on the \textsf{GitHub} benchmark}
    \label{fig:latency-comp}
\endminipage
\end{figure*}


\textbf{Synthesis Quality.}
Figure~\ref{fig:acc-comp} and Figure~\ref{fig:mrr-comp} 
show detailed comparisons of 
accuracy and MRR, between different 
methods on the \textsf{GitHub} benchmark.
Test pipelines are bucketized into 7 groups based on their
lengths (shown on the x-axis), with longer pipelines being
more difficult to synthesize. It can be seen
that \sjrl{} and \sjs{} are comparable in terms of quality,
with \sjrl{} being slightly better in terms of MRR. We can see
that \sjrl{} is noticeably better than \sjsl{}, showing the benefit of
using RL to proactively select
examples to learn from.  

All \sj{} variants are substantially better 
than \textsf{QBO} and \textsf{SQL-by-example} baselines. 
We note that \textsf{SQL-by-example} fails to synthesize
any pipeline longer than 3-steps within our 1 hour timeout limit, 
showing its limited efficacy when dealing with 
large input tables from real pipelines.

\textbf{Latency.}
Figure~\ref{fig:latency-comp} shows a comparison of the
average latency to successfully synthesize a pipeline between all methods
on the \textsf{GitHub} benchmark. While all \sj{} methods have
comparable latency, \textsf{SQL-by-example} 
requires 20x-7x more time to synthesize pipelines up to 3 steps.


\textbf{Pipeline simplification.} We observe that
our synthesized pipelines can sometimes be simpler (with a fewer
number of steps) than human-authored ground-truth 
pipelines, but still being
semantically equivalent. Figure~\ref{fig:ppl-sim}
shows a real example from GitHub, where 
the human-authored pipeline would 
group-by on column \texttt{Gender} for four times with 
different aggregation, %(\texttt{mean}, 
%\texttt{count}, \texttt{median}, \texttt{max}),
before joining them back. 
A synthesized pipeline from \sj{} is a one-liner in this
case and more succinct. While this example
is intuitive, there are many more involved examples of
simplifications (e.g., having an Unpivot on 
each of K similar files followed by (K-1) union, is equivalent to
a Join between the K similar files 
followed by one Unpivot, etc.).

Out of the 700 pipeline in the
\textsf{GitHub} benchmark, our synthesized pipelines are
simpler on 90 cases (12.85\%).
Pipeline simplification is an interesting use case and
an added benefit of \sj. %and even ``semantic translation''
%from one language to another (e.g., from SQL to Pandas).

    \begin{figure}[h]
        \centering
        \subfigure[A human-authored pipeline]{ 
\vspace{-2mm}
            \includegraphics[width=\columnwidth]{figures/ppl_l7.pdf}
            \label{fig:beforeSim}
            }
        \subfigure[A synthesized and equivalent pipeline with fewer steps]{ 
            \includegraphics[width=\columnwidth]{figures/p7_simplified.png}
            \label{fig:afterSim}
            }
        % \includegraphics[width=\columnwidth]{figures/ppl_l7.pdf}
        \caption{An example pipeline simplified after synthesis.}
\vspace{2mm}
    % to be replaced by real results
        \label{fig:ppl-sim}
    \end{figure}




\subsection{Sensitivity Analysis}

\begin{figure*}
\vspace{-13mm}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/latency-t-crop.pdf}
    \caption{Latency by search width $K$.}
    \label{fig:latency-window}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/acc-trend.pdf}
    \caption{Quality by search width $K$.}
    \label{fig:acc-window}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/topk-trend.pdf}
    \caption{Quality by varying parameter choices M (on length-4 pipelines).}
    \label{fig:topk}
\endminipage
\end{figure*}

\textbf{Varying Search Width $K$.} As discussed in
Section~\ref{sec:diversity_search}, 
our search uses a form of beam search by
picking top-$K$ most promising partial pipelines 
in \textsf{GetPromisingTopK()} to reduce the search space.
We perform a sensitivity analysis to study the effect of varying $K$
(from 3 to 24 with a step size of 3)
on synthesis quality and latency.
Figure~\ref{fig:latency-window} shows that 
latency increases roughly linearly with 
$K$, which is expected. It is encouraging to see
that the slope of increase is not significant.
Figure~\ref{fig:acc-window} shows the accuracy with a larger $K$.
We can see that the accuracy plateaus quickly after $K$ reaches 12,
suggesting that our algorithm is effective in picking out 
promising partial candidates with a small $K$.




\textbf{Varying single-operator top-M parameter choices.}
Recall that in \textsf{AddOneStep()}
(Section~\ref{sec:addonestep}),
we consider top-$M$ parameter choices for each 
possible operator when extending partial pipelines.
 We evaluate in Figure~\ref{fig:topk}
the effect of varying $M$ (from 1 to 8).
It can be seen that we get better
accuracy from $M=1$ to $M=2$ 
(because sometimes the desired parameter choice is
ranked at top-2),
but slightly worse MRR (because ranking becomes more difficult
with more candidates). We observe no accuracy/MRR improvement
beyond $M=2$, suggesting that the single-operator 
parameter predictions from \cite{auto-suggest} are fairly reliable, 
with the correct choice consistently ranked among the top-2.

%we run the search-based alogrithm on pipelines of length 4 with different top k  paramters range from 1 to 8. 

\textbf{Varying input table sizes.}
We sample 10 pipelines from the \textsf{GitHub} benchmark
with input tables that have over 100k rows. 
We down-sample their largest input table to 
100k, 10k, 1k, and 100 rows, respectively, and
run synthesis to understand how input sizes
influence synthesizing latency. 
Figure~\ref{fig:table-size} shows that the latency of
our synthesis increases relatively slowly compared to input row --
as the input size increases by 1000x, our latency increases by 3x, 
suggesting that our synthesis has good scalability on large tables.



\begin{figure*}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/size-trend.pdf}
    \caption{Latency by input table sizes on same pipeline tasks.}
    \label{fig:table-size}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/data-size-l5.pdf}
    \caption{Accuracy results by training iterations (on length-5 pipelines)}
	\label{fig:acc-iteration}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/data-size-l5-mrr.pdf}
    \caption{MRR  results by training iterations (on length-5 pipelines)}
	\label{fig:mrr-iteration}
\endminipage
\end{figure*}



\textbf{Varying the number of training iterations.}
For learning-based methods \sj, we 
report in Figure~\ref{fig:acc-iteration} and Figure~\ref{fig:mrr-iteration}
the accuracy/MRR with different numbers of training iterations. 
As can be seen,
both results become fairly stable after
10 iterations. The average execution time 
is about 28 minutes per iteration.




\subsection{Ablation Studies}
To understand the importance of key components
in \sj, we perform ablation studies
in Figure~\ref{fig:ablation-accuracy}.

\textbf{Without FD/Key constraints.}
Recall that FD/Key constraints inferred from output-schema
are key properties we leverage in \sj{} to drastically
reduce the search space. 
The yellow bars in Figure~\ref{fig:ablation-accuracy}
show that without  these constraints, 
accuracy drops consistently.



\begin{figure}
\minipage{0.23\textwidth}
  \includegraphics[width=\linewidth]{figures/ablation-acc.pdf}
    \caption{Ablation study.}
	\label{fig:ablation-accuracy}
\endminipage\hfill
\minipage{0.23\textwidth}
  \includegraphics[width=\linewidth]{figures/error-analysis.pdf}
    \caption{Error Analysis.}
	\label{fig:error-analysis}
\endminipage
\end{figure}





\textbf{Without column-mapping}.
When column-mapping between input/output columns are
not leveraged, it is not possible to estimate 
``progress'' in terms of column coverage, and not possible 
to leverage FD/key constraints (since column-mapping is a prerequisite).
The green bars show a more significant drop in quality.

\textbf{Without single-operator probabilities.}
Finally, when the top-K choices from single-operator models
are used but their probability scores are withheld,
the red bars suggest a modest drop in accuracy.
%This indicates that the FD/key constraints serve as
%important constraints to greatly reduce the feasible solutions,
%making the ranking of candidates from single-operator probabilities
%less critical.

%\todo{Ablation, (optional) without using attribute-names in schema-matching?}

\subsection{Error Analysis}
We analyze cases for which 
\sj{} fails to synthesize correctly. 
Figure~\ref{fig:error-analysis} shows
fail rates, using a breakdown based on whether FD/keys
can be discovered from the target table $T^{tgt}$. 
We can see from the two rightmost bars that
when only FDs can be discovered (key columns are missing), 
or when both FD/keys are missing, fail-rates go up significantly,
which is the main reason for failed synthesis. 

Figure~\ref{fig:error-pipeline} shows an example pipeline with 
the same steps as in Figure~\ref{fig:by-target-intuition}, 
except that the \val{Gender} column is dropped
from the result table in the end. Note that as a result, we could not
discover the FD (\val{Gender} $\rightarrow$ \val{Avg-survived})
from the result table, making it difficult to predict
how the new column \val{Avg-survived} should be generated.
The synthesis problem becomes under-specified, and difficult to get right.
\begin{figure}[h]
\vspace{-2mm}
  \centering
  \includegraphics[width=1\columnwidth]{figures/error-pipeline.png}
  \caption{Example of failed pipeline}
\vspace{-2mm}
  \label{fig:error-pipeline}
\end{figure}


==> response-letter.tex <==
%!TEX root = main.tex

\begin{center}
%\vspace{-12mm}
    {\LARGE Revision for VLDB '21: Auto-Pipeline: 
Synthesize Data Pipelines By-Target}
\end{center}

%{\color{orange}
%Or, is $\widehat{L}(\text{test\_0.csv, test\_1.csv,} \ldots) \stackrel{?}{=} $L(\text{test\_0.csv, test\_1.csv,} \ldots)}

%{\color{orange}
%$\widehat{L}(\mathbf{T}^{in}) \stackrel{?}{=} L(\mathbf{T}^{in})$.}

We would like to thank all reviewers for their constructive feedback. 
We believe addressing these comments indeed improves our paper.


%\vspace{-3mm}
\bigskip
{\huge \stitle{Response to Meta-Reviewer}}
%\vspace{-3mm}

\bigskip
\begin{tcolorbox}
\textbf{1. Clarification of several aspects, e.g.,
what common Python DataFrame operators are supported (R2D1)
role (and limitations) of current constraints discovery and schema matching tools (W3D8/9)}
\end{tcolorbox}


\stitle{Response.}
We have added these clarifications in our revised paper,
as suggested by the reviewers. 

For R2D1, we have added explanations that we select
common DataFrame operators based on a profiling of
real GitHub pipelines we harvested, which identifies
operators that are common in real data pipelines.
We added an analysis of operators
in these pipelines in \rev{Figure~\ref{fig:distributions}},
which shows that a significant fraction of operators 
invoked in real pipelines are indeed supported in our DSL. 

For the specific example of Transpose -- while is not explicitly included
in our DSL, it is actually semantically equivalent to 
invoking an Unpivot followed by Pivot. We have provided
a concrete example in our response to R2D1 to illustrate this point.
We have also added
a test case for synthesis 
using \sj{} to show that a Transpose operator can indeed
be successfully synthesized using our system by
composing Unpivot and Pivot.

For R3D8/9, the reviewer raised a very good question of whether
Key/FD constraints and schema mapping can be reliably inferred
using existing tools, without human intervention. 
We have added a detailed error analysis
(in \rev{Section~\ref{sec:error}}), by sampling 70 failed
cases (10 for each pipeline length group) and manually
analyzed the root cause of these failed cases. We found that
2 out of the 70 cases fail due to spurious FDs,
3 out of the 70 cases fail due to missing Key columns
(dropped in the final steps of the ground-truth pipelines),
and 0 fail due to incorrect mappings (we do remember seeing
failed cases due to incorrect schema-mapping when testing
our system during its development --
such cases are just not represented in this sample of 70 failed cases).

Based on this analysis, we believe that 
inaccurate FDs/Keys/Column-mappings do not contribute significantly to 
why we fail to synthesize pipelines.
We believe this is because
our test pipelines operate on
real data tables (e.g., from Kaggle) that are typically large
(e.g., on average an input table used in 
GitHub pipelines has over 4K rows, and an output
table has over 41K rows). Given that
these tables are fairly large with real and diverse
data content, we find the constraints that can be inferred 
tend to be more reliable (compared to ones discovered
from small synthetic tables, which are more likely to be spurious).  

In order to validate this hypothesis, we perform another
test. We randomly sample 70 test cases (again 10
per pipeline-length group) that \sj currently synthesizes
successfully. We then down-sample the target tables in
each of these 70 cases to 20 rows only, and we then re-run \sj.
We observe that 37 out of the 70 (previously successfully) 
cases would then fail 
due to spurious FDs/Keys, which we believe
confirms our hypothesis that large realistic 
tables indeed allows constraints to be inferred reliably,
making it less of an issue in our setting because we expect
users to point us to large and real data tables as target output
(as opposed to small and synthetic examples that they have
to manually provide by hand, as is often required in
by-example synthesis).

Regarding schema-mapping, we also provided four reasons why 
 it is fairly reliable in our settings in our response to R3D9. We invite
reviewers to inspect our detailed response there.

We do fully agree with the reviewer, however, that relying on Key/FD/column-mappings can be a limiting factor of our 
proposed system, which will likely
fail to synthesize when the target table lacks such constraints for example.
We have highlighted this as well as other
limitations of our system in a ``Limitation of Auto-Pipeline''
section in \rev{Section~\ref{sec:sketch}}.



\bigskip
\begin{tcolorbox}
\textbf{2. Applicability and limitations. The solution relies on good knowledge of the input and the target, this is an important assumption that must come clearly from the first part of the paper. Authors should also clarify better the limitations of the proposed solution. (R1D6, R2D2, R3D1/D2/D7)}
\end{tcolorbox}


\stitle{Response.}
We thank the reviewers for the feedback. We have now added
discussions in \rev{Section~\ref{sec:sketch}} to explicitly describe
these limitations and assumptions.

The key limitations we can identify in our proposed
system include the following:
\begin{itemize}[leftmargin=*]
\item[] (1) Our approach relies on the existence of a table or dashboard that looks like the output users want to generate (e.g., when users want 
to integrate new data into existing database tables or dashboards). In some cases (e.g., when users are truly building a database table or dashboard for the first time, and there is no existing resources to leverage), there may be no such target schema to refer to, making our approach inapplicable. In such cases, users would have to fall back to 
alternative (and more costly) paradigms like program-by-example.
\item[] (2) While our DSL is already fairly general and can cover a large variety of real data pipelines on GitHub, it is not intended to be comprehensive to cover all possible transformation logic.
For example, it does not cover ad-hoc user-defined custom
functions (beyond the string transformations we support), and does not currently handle numeric-calculations, time-series or window-based transformation functions (which are numeric in nature and are infer from schematic examples, thus not included in our DSL).
\item[] (3) While most real pipelines in our benchmarks do have Key/FD constraints that we can leverage to guide our synthesis to find the desired
pipelines, there are a small fraction of test cases (5 out of 70 cases analyzed) where Key/FD constraints are missing (e.g., because the Key columns are dropped in final steps of the pipelines), or unreliable (e.g., because of spurious FD constraints). Pipelines like these are clearly challenging for our by-target
synthesis, given that we do not have paired input/output examples to leverage (as in by-example program synthesis), and will likely fail
using \sj.
\end{itemize}

In addition to listing these limitations in \rev{Section~\ref{sec:sketch}},
we have responded to the questions in
R1D6, R2D2, R3D1/D2/D7 in more detail below, and 
we ask the reviewers to
inspect our responses there for more information.




\bigskip
\begin{tcolorbox}
\textbf{3. Literature. Please position the paper wrt recent relevant approaches. (R1D7)}
\end{tcolorbox}


\stitle{Response.} 
We thank the reviewer for pointing out this very interesting
recent work in R1D7. 
We have cited this related work in our paper, and added an experimental
comparison with this approach in \rev{Table~\ref{tab:overall-github}}
and \rev{Table~\ref{tab:overall-commercial}} of our revised paper.




\bigskip
\begin{tcolorbox}
\textbf{4. A more realistic experiment would be great, also to address/reply to point 2 above. For example, authors can test a setting where they introduce more (e.g., irrelevant) sources to see when the search space brings everything to a grinding halt, introducing some confounding factors into the sources (e.g. representational inconsistencies) to see what happens to the quality, or just providing sources that are quite poor for populating the target - how does the system acts with a less-than-ideal situation?}
\end{tcolorbox}


\stitle{Response.} 
While we already use real data pipelines as test cases for evaluation,
we do agree with the reviewers that testing the behaviour of
our system in a less-than-ideal situation (e.g., with noisy/irrelevant
data files, data columns, and data values) would be 
a very good idea.

We have performed new experiments exactly as suggested
in this meta-review comment, and added 
a new section dedicated 
to the robustness of our system in \rev{Section~\ref{sec:robustness}}
of our revised paper. Specifically, we tested 
(1) when $K$ irrelevant input tables (sampled from
other irrelevant pipelines) are added as
noise into each test case; (2) when $K$ irrelevant
data columns (sampled from other irrelevant pipelines)
are added as noise into each input table of each test case;
and (3) when $p$ fraction of data values in randomly sampled columns
are perturbed/scrambled. 


We would like to report that our new 
results suggest that \sj{} is
indeed robust to these different types of injected noises.
Detailed data can be 
found in \rev{Figure~\ref{fig:table-robust}, \ref{fig:column-robust},
and \ref{fig:perturb-robust}} of our paper.

We hope these new robustness tests in less-than-ideal
situations can address the concerns raised 
in meta-review \#2 and \#4.


%\vspace{-3mm}
\bigskip
{\huge \stitle{Response to Comments by Reviewer 1}}
%\vspace{-3mm}

\bigskip
\begin{tcolorbox}
\textbf{D1. Figure 3. It is good to have this running example, but the synthesized pipeline is essentially the same as the original. A more interesting example would have faced a more significant challenge.}
\end{tcolorbox}

\stitle{Response.} The reviewer is correct that we made this running 
example in Figure 3 simple for ease of understanding. In practice
when synthesizing real pipelines from GitHub, we 
see more challenging cases where the synthesized pipelines would
look substantially the human-authored pipelines, like suggested in the comment.

To better quantify this effect, we analyzed 700 real pipelines in our
GitHub benchmark, and found for 90 cases (12.85\%), our synthesized
pipelines are significantly ``simpler'' 
(with less number of pipeline steps) than the human-authored pipelines,
with the synthesized pipelines still
being semantically equivalent to the human-authored ones. 
To better illustrate this, we now 
give a concrete example of such a pipeline 
in \rev{Figure~\ref{fig:ppl-sim}}, which explains a 
real pipeline authored by humans, and a corresponding pipeline
synthesized by our algorithm that is significantly simpler/different.

We believe this demonstrates that 
our synthesis algorithm is not just ``mimicking''
human experts when learning from training pipelines, 
it actually explores the search space and
finds more efficient (measured by number of steps) ways
to synthesize pipelines (sometimes not obvious to humans), which
we believe is indeed a challenging task.
(Just to be sure, the synthesis algorithm does not get to see the 
test pipelines authored by humans, during either training or testing,
so even being able to ``mimic'' human behaviors in this case is no small challenge). 

We have expanded our discussion 
in \rev{Section~\ref{sec:comparison} and Section~\ref{sec:target}} to better explain this point, using a concrete example (\rev{Figure~\ref{fig:ppl-sim}}) as suggested.



\bigskip
\begin{tcolorbox}
\textbf{D2. Section 2.3. The objective places high expectations on the target, and the consistency of the sources with the target. The expectation includes that the Keys and FDs are known, and also preserved when there may be unreliable or inconsistent input data. It would be good to revisit these expectations explicitly in the experiments (though see W1).
\\
W1. Perhaps the experimentation is focused on an unrealistic case, assuming good knowledge on both the inputs and the outputs.}
\end{tcolorbox}

This is an important topic worth more discussion. 
First of all, we should note that our test 
pipelines are all real ones authored by
human experts, which we programmatically crawled from GitHub.
The input tables of these pipelines are 
typically real data (e.g. Kaggle datasets),
many of which have known quality/consistency issues
(a search of ``data cleaning'' on Kaggle returns over 
51K results\footnote{\url{https://www.kaggle.com/search?q=data+cleaning}}). 
On the output side, we similarly have no control over the
output tables, as they are programmatically generated
from given input tables, using pipelines authored by humans.
So for both input and output tables are
real test cases, which are not curated or cleaned in 
to make them easier to synthesize, which we
now highlight in \rev{Section~\ref{sec:dataset}}.

Despite the fact that we are using real data and real pipelines
as test cases, it would indeed be interesting to test the robustness
of our synthesis algorithm when we inject additional ``noise''
into the test cases in a controlled manner, like suggested.
We have performed new experiments and added 
a new section dedicated 
to robustness in \rev{Section~\ref{sec:robustness}}
of the revised paper. Specifically, we tested 
(1) when $K$ irrelevant input tables (sampled from
other irrelevant pipelines) are added as
noise into each test case; (2) when $K$ irrelevant
data columns (sampled from other irrelevant pipelines)
are added as noise into each input table of each test case;
and (3) when $p$ fraction of data values in randomly sampled columns
are perturbed/scrambled. 

We would like to report that our new 
results suggest that the \sj{} algorithm is
indeed robust to these different types of injected noises.
Detailed data can be 
found in \rev{Figure~\ref{fig:table-robust}, \ref{fig:column-robust},
and \ref{fig:perturb-robust}}, and discussed in 
\rev{Section~\ref{sec:robustness}}.

The reviewer also raised an interesting question about Keys
and FDs, on whether they are known, and how reliably
we can rely on them for synthesis.  In our work, we do not
require users to declare Keys/FDs, instead we use
standard Key/FD discovery algorithms from the literature
to discover them (e.g.,~\cite{buranosky2018fdtool}).
It is however, an important question as to whether these
discovered Keys/FDs are reliable enough 
for synthesis to succeed
(it is known that some discovered FDs may be spurious false-positives). 

To answer that question, we performed a detailed
error-analysis of in \rev{Section~\ref{sec:error}}. Specifically,
we sample 70 failed test cases (10 cases for pipelines
in the same length-group), and categorize the
failed cases by their root causes. Only 2 out of the 70 cases
fail due to spurious (false-positive) FDs, and 3 are due to missing keys.

We believe
the key reason why spurious constraints are not 
a significant issue in our evaluation, is because 
our test pipelines operate on
realistic data (e.g., Kaggle tasks) with large tables
(e.g., on average we have over 4K rows per input table,
and over 41K rows per output table). Such large tables make
false discovery of spurious constraints substantially less likely. 
In order to better illustrate this point, we sample
70 test cases that \sj{} can currently synthesize successfully.
We then down-sample their target 
tables to 20 rows each.  When we re-run our synthesis algorithm, 
we observe 37 out of 70 
cases would then fail due to spurious FDs/Keys,
confirming our hypothesis that having large realistic 
tables indeed prevents spurious constraints from being
discovered. 

We have added these new results in our revised paper, and
we invite the reviewer to inspect the corresponding sections
in the paper for more details.


\bigskip
\begin{tcolorbox}
\textbf{D3. By Section 3.1 and 3.2, the same information has been provided several times at much the same level of detail. It would have been better to avoid this repetition, and to say a bit more about what is going on in [47].}
\end{tcolorbox}


\stitle{Response.} We have revised these two sections accordingly and we
thank the reviewer for the suggestion. 


\bigskip
\begin{tcolorbox}
\textbf{D4. As [47] is being used to choose the next step, but [47] knows nothing about the target, this seems to be forward chaining, where backward chaining could help to focus the search.}
\end{tcolorbox}

\stitle{Response.} This is a very interesting way to look at [47], relative
to the new by-target synthesis problem we propose in this work.
Indeed [47] is intended to select the best local 
operator for this step that users try to add in their pipelines.
The problem in [47] is substantially easier than
the multi-step synthesis problem we study, which
requires looking ahead much further (sometimes for 10 or more
pipelines steps).

We should note that while the backward chaining analogy is very
attractive at a conceptual level, it is not something easy to realize
on top of [47].  For example, given an output table with 10 rows that is 
the result of an groupby/aggregation step, it is hard to reverse-engineer
for even \textit{one step}, to
reasonably predict what the input should look like, or exactly
what groupby/aggregation has been performed on that input 
in order to produce this observed output table (e.g., what
aggregation operators are used). Imagine that we have a data pipeline with
10+ steps like in the GitHub benchmark 
we study -- it is not hard to see that reserve-engineering 
 \textit{multiple steps} from
the output backward would likely not get us too far, given that
we could not even reliably reserve-engineer one-step, 
and additional predictions would critically depend on the inferences
from previous steps.

Because of the difficulty of realizing backward chaining
in a reliable manner, we could not 
easily extend [47] backward to make it work in our setting.
However, during revision, we did further expand our evaluation,
by comparing two more additional methods, 
Auto-Pandas~\cite{bavishi2019autopandas}, which is 
a recent ``by-example'' method that utilizes Graph Neural Networks
(GNNs), and end-to-end data wrangling~\cite{koehler2019incorporating},
which utilizes data contexts including table schema. 
These are additional methods that do consider the ``target'' 
and can be considered as a form of ``backward chaining''. We
 invite the reviewer to inspect these new results 
in \rev{Section~\ref{sec:experiments} (Table~\ref{tab:overall-github}
and Table~\ref{tab:overall-commercial})} for details. 

\bigskip
\begin{tcolorbox}
\textbf{D5. I didn't fully understand the representation. Figure 8 is abstact, and perhaps providing a concrete example would help. The experiments make a clear claim that the evaluation is with unseen sources and flow components, which is good. However, it is not clear to me how the state generalises from the details of an individual pipeline.}
\end{tcolorbox}


\stitle{Response.}
We thank the reviewer for the comment, and have updated our
running example in \rev{Section~\ref{sec:learning}} to better clarify 
the intuition behind our deep model in Figure~\ref{fig:model}.

The reason this architecture and state representation generalize
beyond individual pipelines, is that we explicitly encode 
``progress'' made by intermediate steps of 
partial pipelines, in achieving the target Keys/FDs/Operators/Mappings.
Specifically, if we look at Figure~\ref{fig:model}, on the left
side, each section corresponds to one type of information we
would like to capture -- e.g., the lower-left is for FDs, the 
section above it is for operator probabilities, and the section further
up is for Key constraints, etc. 
Let us narrow in on one section, the lower-left part for FDs 
(other sections for Keys/Mappings/Operators are modeled similarly). 
We can see that here, each row corresponds to an FD
discovered from the target table that we need to satisfy, marked
as FD-1, FD-2, etc., in the figure. Each column 
corresponds to a partial pipeline created at time-step, marked as
$T$, $T-1$, etc. Each of these partial pipelines is one we are 
exploring in the synthesis process, and a partial pipeline with 
$T-1$ is the one immediately precedes the one at time-step $T$
(i.e., with one less operator).

This representation makes it easy for 
a convolutional neural network (CNN) to learn
whether we are making progress (achieving FDs
that would be required in the target output).
Specifically, given the convolutional filter shown in the middle
of Figure~\ref{fig:model}, which is hopefully
learned with weights shown on the 
figure (the last two being a ``-1'' and a ``+1''),
then with an element-wise convolution (a standard
step in convolution networks), we produce
a ``+1'' shown in the output that corresponds
to FD-2. It can be verified
that this ``+1'' output is only possible when the
bit corresponding to FD-2 is 0 at time-step $T-1$,
which is then flipped to ``+1'' at $T$, which
corresponds to our intuitive notion of ``making progress''
in achieving one additional FD that would be required 
in the target (suggesting that our partial pipeline is likely
moving in the right direction).

It is easy to see that while this example above is only for FD,
it translates easily to other types of information captured 
in other sections of the model in Figure~\ref{fig:model}
(Keys, Operators, Mappings, etc.). Overall, these
individual progresses are combined and weighted in
final layers of the model, to make an aggregate
prediction of whether a partial pipeline is promising
in realizing all constraints required in a correct synthesis. 
It can be seen that all of these considerations 
(making progress in FD/Key/Operator/Mapping) are not specific to 
one individual pipeline, but generalizes across all synthesis
cases. 

We hope these details would explain our intuition behind our model/representation a little better now, and invite the reviewer to
read our revised \rev{Section~\ref{sec:learning}} for more details.


\bigskip
\begin{tcolorbox}
\textbf{D6. Section 5.4. The experiments sound quite general. However, it seems that the question that is really being asked is the following: Given the suitable inputs and the correct output, synthesize a program for getting from the former to the latter. This assumes that a lot is known about the output and the most suitable inputs. What if we do not know the most suitable input? What if we know less about the output? The applicability of the proposal needs to be discussed more clearly. }
\end{tcolorbox}


\stitle{Response.}
This is a good question, and related to comment D2 above. While our problem setup is general (given input/output tables, infer a synthesized 
program from the former to the latter), our unique insight is that by (1) focusing on a small DSL with common
table-manipulation operators (listed in Figure~\ref{fig:DSL} of the paper), 
and (2) leveraging inferred constraints such as Keys/FDs, we can
constrain the search space significantly and make the overall problem
tractable. This is not something that has been explored/understood from
the prior work, and we find this to be an interesting new direction
for future work.

Regarding the question of what is assumed to be known about the
output and inputs -- we have added various new experiments  to test the robustness of our system, and
we ask the reviewer to kindly inspect our response to D2 for details.
As a brief summary here, on the input table side, we added experiments (in \rev{Section~\ref{sec:robustness}}) to show that
the success rate of our synthesis holds up fairly well even when
(1) additional irrelevant input tables are intentionally injected
into synthesis tasks, (2) additional irrelevant data columns
are intentionally injected into input tables, and (3) data values
in input columns are intentionally altered to create noisy
data values.

On the output side, we added detailed error analysis
(\rev{Section~\ref{sec:error}}) to show that false discovery
of FDs/Keys do not contribute significantly to failed synthesis
(only 2 out of 70 are in this category).
This is because even though spurious discovery of FDs and keys 
from small input tables
is a known issue~\cite{papenbrock2016hybrid}, 
our test pipelines operate on
real data tables (e.g., from Kaggle) that are typically large
(e.g., on average an input table used in 
GitHub pipelines have over 4K rows, and an output
table has over 41K rows), such that constraints can be inferred reliably from
these tables.  When we down-sample our target tables
of each test case to 20 rows each and re-run \sj,
we observe 37 out of 70 
cases would then fail due to spurious FDs/Keys,
confirming the hypothesis that large realistic 
tables indeed allows constraints to be inferred reliably.

We do agree with the reviewer that the effectiveness
of our approach critically depends on these constraints
to be inferred from input/output tables, which can be a
limitation (e.g., when Key/FDs are absent in target tables).
We added a section dedicated to ``Limitation of Auto-Pipelines''
in \rev{Section~\ref{sec:sketch}}, which we hope would better
clarify these questions regarding applicability and assumptions.

\bigskip
\begin{tcolorbox}
\textbf{D7. The following paper also describes an end-to-end data preparation system that builds on information about the target: Martin Koehler, Edward Abel, Alex Bogatu, Cristina Civili, Lacramioara Mazilu, Nikolaos Konstantinou, Alvaro A. A. Fernandes, John A. Keane, Leonid Libkin, Norman W. Paton: Incorporating Data Context to Cost-Effectively Automate End-to-End Data Wrangling. IEEE Trans. Big Data 7(1): 169-186 (2021)}
\end{tcolorbox}


\stitle{Response.}
We thank the reviewer for bringing our attention to 
this paper (it was published really recently
in March 2021, which we would have missed
without your help). We have cited the paper
and added discussions for this very interesting approach.

Because the code associated with this paper is not yet publicly
available for comparison, we added an experiment to compare
\sj{} with 
the theoretical upper-bound coverage of this alternative
system, by treating all test pipelines whose operators are
covered by the DSL of this alternative approach as ``successes''
(thus giving an upper-bound of the fraction of pipelines that
can be synthesized using the alternative method).
Our new results in \rev{Section~\ref{sec:experiments}
 (Table~\ref{tab:overall-github}
and Table~\ref{tab:overall-commercial})} suggest that 
the accuracy of \sj{} is quite a bit higher than
the theoretical coverage of this alternative method.
We invite the reviewer to inspect these new results 
in our revised paper.





%\vspace{-3mm}
\bigskip
{\huge \stitle{Response to Comments by Reviewer 2}}
%\vspace{-3mm}

\bigskip
\begin{tcolorbox}
\textbf{W1. It is not clear why all "common" data operators are supported, such as transpose.
\\
D1. It is not clear whether all common Python DataFrame operators are supported, e.g., transpose. }
\end{tcolorbox}


\stitle{Response.}
This is a great question worth discussing. We indeed aspire
to cover most if not all common data operators, and
our DSL (in Figure~\ref{fig:DSL}) is designed based on
the common operators profiled from
real GitHub pipelines. We added an analysis 
in \rev{Figure~\ref{fig:distributions}} to show that most operators
in our GitHub benchmark 
would indeed be covered in our DSL.

Transpose is a really interesting example -- 
while technically it is not in our DSL, 
as rightly pointed out by the reviewer, 
it is actually equivalent to invoking an Unpivot (called Melt in Pandas
terminology), followed by a Pivot. This semantic equivalence
is known and documented (e.g., \url{https://stackoverflow.com/questions/15297809/sql-transpose-full-table} and \url{https://stackoverflow.com/questions/13372276/simple-way-to-transpose-columns-and-rows-in-sql}).

Given this equivalence, introducing Transpose into the
DSL will not enhance the expressiveness of the pipelines we can synthesize,
because a Transpose operation can be equivalently synthesized
using a Unpivot and a Pivot. 

In order to demonstrate this point,
we produce a standard test case of transpose, shown 
in Listing~\ref{transpose} below\footnote{adapted
from Pandas documentation~\url{https://pandas.pydata.org/docs/reference/api/pandas.DataFrame.transpose.html}}. 


\begin{lstlisting}[language=Python, caption=An example pipeline that performs transpose, label=transpose]
import pandas as pd
d1 = {'index': ['row1', 'row2'], 'col1': [1, 2], 'col2': ['a', 'b']}
df1 = pd.DataFrame(data=d1).set_index(['index'])
df2 = df1.T
\end{lstlisting}

The input/output table of this test case can be seen
from Figure~\ref{fig:transpose-1} and Figure~\ref{fig:transpose-2},
respectively.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\columnwidth]{figures/transpose-1.png}
    \caption{Input table for transpose}
\label{fig:transpose-1}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\columnwidth]{figures/transpose-2.png}
    \caption{Output table for transpose}
\label{fig:transpose-2}
\end{figure}

When we feed such a test case to \sj, our system can successfully 
synthesize a semantically equivalent pipeline with 
an Unpivot (called Melt in Pandas) followed by
a Pivot, like shown in Listing~\ref{transpose2} below, 
which is equivalent to a Transpose.

\begin{lstlisting}[language=Python, caption=Synthesized transpose using Unpivot and Pivot, label=transpose2]
import pandas as pd
d1 = {'index': ['row1', 'row2'], 'col1': [1, 2], 'col2': ['a', 'b']}
df1 = pd.DataFrame(data=d1)
df2 = pd.melt(df1, id_vars=['index'], value_vars=['col1','col2'])
df2.pivot(index='variable', columns='index')
\end{lstlisting}

While our DSL does covers Transpose as a result, 
there are additional transformations that are 
not currently covered in our DSL (e.g., window-operations).
These transformations are numeric in nature and
more challenging to predict correctly, 
which are thus not included in our DSL (or the DSLs used
by previous by-example systems).
The reviewer is correct that extending to these additional operators
would indeed be useful future work, which we have added
as a limitation in \rev{Section~\ref{sec:sketch}}, and also a
potential direction for future work in \rev{Section~\ref{sec:conclusion}}.

\bigskip
\begin{tcolorbox}
\textbf{W2. The target is only a schema or any possible extensions?
\\ 
D2. Currently, by-target is mainly a target schema. This is simple and good. However, are there any other similar "simple" targets that users can easily specify?}
\end{tcolorbox}

\stitle{Response.}
The reviewer is absolutely correct that extending our current
specification with additional feedback that users can provide
would also be interesting directions for future work.
For instance, when column headers are cryptic and identifying
column mappings becomes challenging,
we envision a user-experience where users can optionally
provide feedback, either using a graphical user interface to identify
mappings (similar to ones used
in schema mapping systems), or entering matching 
column names for input/output tables so that the mapping
becomes straightforward.

We added some discussions along these lines in \rev{Section~\ref{sec:conclusion}}, and we thank the reviewer for the suggestion.

\bigskip
\begin{tcolorbox}
\textbf{D3. If one missing operator is considered as a small piece of code, there is a recent related work "Searching a Database of Source Codes Using Contextualized Code Search" in VLDB 20. It is interesting to have a discussion about whether their approach can help in auto-pipeline.}
\end{tcolorbox}



\stitle{Response.}
Code search is indeed a related area of research.
We have added this related work in \rev{Section~\ref{sec:related}} 
of our paper, and some discussions
around this topic in general. We feel that in our specific problem
of pipeline-by-target, our problem specification mostly come from
the input/output data. Unlikely contextualized code search,
when we start our synthesis 
we have an empty pipeline with no code 
snippets to leverage, and it is mostly the characteristics of
data (relative to our target output) 
that guide us to find the correct synthesis. 

Nevertheless code search is an interesting and relevant line
of work worth mentioning. We have added these discussions
as suggested.



%\vspace{-3mm}
\bigskip
{\huge \stitle{Response to Comments by Reviewer 3}}
%\vspace{-3mm}



\bigskip
\begin{tcolorbox}
\textbf{D1. The paper is quite interesting but seems to make strong assumptions to work.}
\end{tcolorbox}

\stitle{Response.} We thank the reviewer for the constructive feedback. We
believe this comment relates to detailed comments like D7, D8, and D9 below. We invite the reviewer to inspect our detailed responses below.

\bigskip
\begin{tcolorbox}
\textbf{D2. It is always helpful to have a summary of contributions in the intro.}
\end{tcolorbox}

\stitle{Response.} We have added a summary of contribution section in 
\rev{Section~\ref{sec:intro}}, as suggested.


\bigskip
\begin{tcolorbox}
\textbf{D3. The paper central assumption is that a user would be able to point to a “schematically similar” target table; (not examples of output for some tuples of the input). The authors should have started with good and clear examples showing various such cases, in different domains, and then take one of these examples to show why their intuition would work.}
\end{tcolorbox}

\stitle{Response.}
This is a good suggestion. We have updated our paper to better
clarify/explain this point.

This by-target paradigm arises from a 
common usage pattern that we observed in ETL and BI
workflows (and confirmed by our colleagues in product teams
like Microsoft Power BI), which is that users often have to 
repeatedly integrate new data files into existing database tables
or BI dashboards,
for example, whenever sales data from a new store/region/time-period
becomes available. However, because the input schema
of these new data files (for new stores/regions/time-periods)
may be different from the existing
input data for which data pipelines have been built,
the new data files cannot be on-boarded using
existing data-pipelines.

Our observation is that in such scenarios, users typically have a 
precise ``target'' in mind, such as an existing database table
or BI dashboard, with a precise goal of bringing the new data into a form 
that ``looks like'' the existing target table (so that the new data
can be integrated/union-ed into existing tables).

We should note that such a scenario of repeatedly
onboarding similar data files
into existing pipelines is not a problem we
dream up, but a common challenge faced by
customers of commercial products like Microsoft Power BI, and
is also documented online by other
commercial vendors (for example, \url{https://www.trifacta.com/blog/goldilocks-solution/} by Trifacta).

We have revised our \rev{Section~\ref{sec:intro}}
and \rev{Section~\ref{sec:problem}} to better explain the
motivations. While our experiments on 700 real GitHub pipelines
show that the by-target approach works reasonably
well when users can provide us with a target table, we do admit 
that our approach would not 
be applicable when such a ``schematically
similar'' table does not exist (e.g., this is the first time
someone needs to build such a pipeline, with no
existing output data to refer to). We have also highlighted this key
limitation/assumption in \rev{Section~\ref{sec:sketch}} of our revised
paper.

\bigskip
\begin{tcolorbox}
\textbf{D4. The next point is to better explain why constraints such as FDs and keys are good enough to guide the synthesis process and the intuition on how this will guide the synthesis process.}
\end{tcolorbox}

\stitle{Response.} This is an important point. We have
updated our discussions and the running example 
in \rev{Section~\ref{sec:target}},
to better explain why constraints like FDs and keys are
often enough to sufficiently constrain the search problem
and guide the synthesis process to successfully find
the desired pipeline. 

A related question is why FDs/Keys inferred from given tables
may be reliably used in our by-target synthesis (D8). We invite
the reviewer to inspect our detailed response to D8 below.

\bigskip
\begin{tcolorbox}
\textbf{D5. Also, how about other profile information such as distribution, domains, patterns, data types, etc. Are these of any use?}
\end{tcolorbox}

\stitle{Response.}
This is a good point. The reviewer is correct that profile
information such as distribution,
domains, patterns, and data types are highly valuable, particularly
 in our schema-mapping
step, for us to identify likely column-to-column mappings,
when two columns that should map have no
data-values in common (e.g., two date-time columns with
disjoint ranges of time-stamps).

The use of these aforementioned signals in the context of column-mapping
has been previously studied in the
schema-mapping literature~\cite{rahm2001survey}.
We indeed make use of all of these signals (which
we mention only briefly in Section~\ref{sec:verifycands}
due to space constraints, and can also be seen
from the code we release for inspection\footnote{\url{https://www.dropbox.com/sh/574gox2waefn5cj/AADxltcc8K_ffFEDew0UPTIDa?dl=0}}.) 

Because what we do 
is not too different from well-known 
schema-mapping techniques in the literature, so given 
the space constraints we decided to trade these off for
new materials/algorithms that are not known in the literature.
We did however, add more details for this part on how we leverage
patterns and distributions  (including the formula used
in our similarity calculation) in a full version
of our paper\footnote{\url{https://www.dropbox.com/sh/574gox2waefn5cj/AADxltcc8K_ffFEDew0UPTIDa?dl=0}}, which we plan to
release on arxiv for readers in the details of the schema mapping step.


\bigskip
\begin{tcolorbox}
\textbf{D6. The proposed system supports simple operations as those described in Figure 5, the authors should discuss cases where the desired transformations involve complex computations and formulas.}
\end{tcolorbox}

\stitle{Response.} 
The reviewer is correct that the proposed system would not
be able to support complex computations and formulas. 
Such operators (e.g., elementary arithmetic operators ``+'', ``-'',
``$\times$'', ``/'') are not included in our DSL (Figure~\ref{fig:DSL})
and not intended to be synthesized. 

We should note that complex computations such as numeric calculations
are generally hard to infer even with paired input/output examples 
(e.g., given an input of ``1'' and an output of ``3'', inferring a 
numeric calculation is typically an under-constrained problem).
As such complex numeric 
computations are typically not considered in the traditional
literature of by-example synthesis as well. By-target synthesis
is even less constrained compared to the by-example paradigm,
making it even less likely that we can correctly synthesize 
complex computations.

We realized that presenting our DSL alone 
may not be enough to make it clear what operators 
are not supported.
We have emphasized this fact more in a 
separate ``Limitations of Auto-Pipeline''
section, which can be seen in the
\rev{Section~\ref{sec:sketch}} of the revised paper.


\bigskip
\begin{tcolorbox}
\textbf{D7. They need to clearly state the limitations of their systems as it seems they are overclaiming what it can do.}
\end{tcolorbox}


\stitle{Response.}
We thank the reviewer for the feedback, and have now added
a paragraph in \rev{Section~\ref{sec:sketch}} 
to explicitly discuss the limitation
of our system. The key limitations we can identify in our proposed
system are as follows:
\begin{itemize}[leftmargin=*]
\item[] (1) Our approach relies on the existence of a table or dashboard that looks like the output users want to generate (e.g., integrating new data into existing database tables or dashboards). In some cases (e.g., when users are truly building a database table or dashboard for the first time, and there is no existing resources to leverage), there may be no such target schema to refer to, making our approach inapplicable and one would have to fall back to related
(but more costly) paradigms such as program-by-example.
\item[] (2) While our DSL is already fairly general and can cover a large variety of real data pipelines on GitHub, it does not cover ad-hoc user-defined custom
functions (beyond simple string transformations that we support), and does not currently handle time-series and window-based transformation functions (which are numeric in nature and are inferred from schematic examples, thus not included in our DSL).
\item[] (3) While most real pipelines in our benchmarks do have Key/FD constraints that we can leverage to guide our synthesis to find the desired
pipelines, there are a small fraction of test cases (5 out of 70 cases analyzed, to be discussed in our response to D8 below) where Key/FD constraints are missing (e.g., because the Key columns are dropped in final steps of the pipelines), or unreliable (e.g., because of spurious FD constraints). Pipelines like these are clearly challenging for our by-target
synthesis, given that we do not have paired input/output examples to leverage, like in the case of by-example program synthesis. 
\end{itemize}

\bigskip
\begin{tcolorbox}
\textbf{D8. Constraint discovery (e.g., FDs, keys, …) seems to be trivialized by the authors. Many of the profiling tools will discover many such constraints and not all of them are meaningful/valid as it is well documented in the literature. In fact, in many cases, a human has to be involved to validate/accept which constraints to consider. The authors should explain how they are dealing with this aspect.}
\end{tcolorbox}

\stitle{Response.} This is a very good point. The fact that existing
 techniques tend to uncover spurious 
false-positives discovery is known in the literature (e.g.
discussed in~\cite{papenbrock2016hybrid}), especially
on small input tables. In our case we depend on the
FDs/Keys discovered automatically, and the question is whether
they can be relied upon 
without human intervention. 

We added a detailed error analysis
(in \rev{Section~\ref{sec:error}}), by sampling 70 failed
cases (10 for each pipeline length group).
We carefully analyzed the root cause of these failed cases, and
categorized them into 4 main categories. We found that
only 2 out of the 70 cases fail due to spurious FDs, and
3 out of the 70 cases fail due to missing Key columns
(dropped in the final steps of the ground-truth pipelines).

Based on this analysis, we conclude that 
inaccurate FDs/Keys do not contribute significantly to 
why we fail to synthesize correct pipelines.
We believe this is because
our test pipelines operate on
real data tables (e.g., from Kaggle) that are typically large
(e.g., on average an input table used in 
GitHub pipelines has over 4K rows, and an output
table has over 41K rows). Given that
these tables are really large with real and diverse
data content, the constraints that can be inferred 
tend to be more reliable (compared to ones discovered
from small synthetic tables).  


In order to validate this hypothesis, we perform another
test. We randomly sample another 70 test cases (again 10
per pipeline-length group) that \sj currently synthesizes
successfully. We then down-sample the target tables in
each of these 70 cases to 20 rows only, and we then re-run \sj.
We observe that 37 out of the 70 (previously successfully) 
cases would then fail 
due to spurious FDs/Keys, which we believe
confirms our hypothesis that large realistic 
tables indeed allows constraints to be inferred reliably,
making it less of an issue in our setting because we expect
users to point us to large and real data tables as target output
(as opposed to small and synthetic examples that they have
to manually provide by hand, as is often required in
by-example synthesis).


We have added these details in \rev{Section~\ref{sec:error}}
of the paper, which we hope can help to address this concern.

\bigskip
\begin{tcolorbox}
\textbf{D9. The same can be said about “standard schema matching” which oftentimes require human intervention to choose the best matches.}
\end{tcolorbox}

\stitle{Response.} Like in Keys/FDs, we indeed do not require
human to intervene and choose the best matches for schema matching.
In our detailed error analysis of 70 failed cases sampled from
our test results 
(in \rev{Section~\ref{sec:error}}), we found 0 cases that
can be attributed to failed schema mappings. However, outside of
these 70 sampled failed cases, and during the development/test phase
of our algorithm, we did remember seeing a couple failed cases from
our 700 case GitHub benchmark that are due to incorrect
column mappings. 

We feel that there are a few reasons why  schema mapping
turns out to be fairly reliable in our test settings. First, 
like in the case of Keys/FDs, our pipelines are operating on relatively large
data tables (e.g., input tables have on average over 4K rows, 
and output tables have on average over 41K rows). With a large
collection of data values between columns in input/output tables,
the chance of having content overlap between source/target columns
after our train/test split is fairly high, making schema mapping reasonable
reliable when we leverage data-instance-based signals. 

Second, for real data pipelines we harvest 
from GitHub, we observe that in a large fraction of 
cases, developers would not modify column names
from input to output, or would only modify them slightly,
making our schema mapping reliable leveraging column-name-based
signals.   

Third, for cases where column
names are modified in the pipeline, 
we find the data-pattern-based signals (e.g., generalizing
date-time strings into regex-patterns) can often
complement the other signals to identify reliable column-mappings
(described in detail in a full version of our paper~\cite{full}).

Fourth, unlike schema mapping in integrating large
enterprise databases that may involve databases
with hundreds or thousands of data columns, in our test cases using
real GitHub pipelines, we find there are on average less than 10 columns
per input file (some of which may not be needed in the result and
dropped from the final output), which may also contribute to the
high success rates we observe from the schema-mapping component.

Finally, the schema mapping we produce is a ``soft'' 1:N mapping
(linking a column from one table to K likely columns to map to 
in the other table
whose similarity is over a fixed threshold). This is unlike 
``hard'' 1:1 column mapping required by standard schema
mapping, where the task is more difficult. 
Note that this soft-mapping gives us a lot flexibility
in ``covering'' columns in the target table -- as long as one of the
columns in our 1:N soft mapping is the correct column mapping,
we have identified the desired mapping and the corresponding pipeline
(and if the soft mapping is incorrect then we have wasted a slot in 
the top-K pipelines we produce, but the task may still succeed with
some of the other pipelines in the top-K).

\bigskip
\begin{tcolorbox}
\textbf{D10. Line (9) Algorithm 1, which involves VerifyCands, is confusing, do all intermediary pipelines need to verify constraints 2, 3, $\&$ 4 from PMPS?}
\end{tcolorbox}

\stitle{Response.}
The reviewer is correct that in Algorithm 1, any final
candidate pipeline we synthesize and return as a top-K 
from Algorithm 1 will have to pass
the checks of constraints 2, 3, $\&$ 4 in PMPS using 
the subroutine VerifyCands (otherwise such a pipeline will
most likely fail and waste a top-K slot).

However, for \textit{intermediate/partial} pipelines explored
by the synthesis algorithm that are not yet the final top-K output,
they do not have to pass the same checks (e.g., some
FD/Keys may still be missing from the intermediate results). 
This is reflected in
Line (8) of Algorithm 1 -- all promising intermediate pipelines
are saved in $S_{depth}$, which is not subject to the verification
of VerifyCands, and will be used for the next iteration of 
finding promising intermediate pipelines (Line 4-8). 
In Line (9), we do invoke 
VerifyCands on these intermediate pipelines $S_{depth}$,
only to save the ones meeting the PMPS requirements in
a separate variable $candidates$, which will be used to 
select the final top-K before we return from Algorithm 1 (in Line 10).

We understand this may be confusing from the pseudo-code alone, and
have updated our description of Algorithm 1 in \rev{Section~\ref{sec:algo_overview}} to make this more clear.

\bigskip
\begin{tcolorbox}
\textbf{D11. What’s the intuition about using a diversity-based strategy for GerPromisingTopK; what would be other choices and why this one is the best?}
\end{tcolorbox}

\stitle{Response.}
We have update \rev{Section~\ref{sec:diversity_search}} of our
revised paper to make the explanation more intuitive. 

The intuition behind the diversity-based search strategy, is that
we want to balance between a number of desirable criteria 
that we want to see in
the partial pipelines we synthesize. Specifically, we want
to have a pipeline such that:

\begin{itemize}[leftmargin=*]
\item[] (1) Its operator invocations are likely with high predicted probabilities;
\item[] (2) Its intermediate results can satisfy as many 
FD/Key constraints discovered from the target table as possible;
\item[] (3) Its intermediate results can
``map'' as many columns in the target table as possible.
\end{itemize}

These 3 criteria may not be simultaneously achieved by the same
candidate pipeline, and we may have a skyline of choices where
different candidate pipelines are better in one of the three different
dimensions.
For example, one candidate partial pipeline $L_1$ may be the
most likely based on predicted operator probabilities; 
a second partial pipeline $L_2$ achieves
a few more FD/Key constraints than any other candidates, while
a third candidate partial pipeline $L_3$ may successfully map
the most number of columns in the target table. 
Since all three criteria are desirable, it is hard to know
which among $L_1$, $L_2$ and $L_3$ is the most desirable/promising
(because the three desirable dimensions are not directly comparable,
making us comparing apples with oranges in this case).

Given the difficulty in comparing candidates among these three
desirable dimensions, for the diversity-based search algorithm,
we simply pick the $\frac{K}{3}$ best candidates along each
of the dimensions, which is really the intuition behind our
diversity-based strategy. (Note that the three considerations
listed above directly correspond to the three criteria listed
in Section~\ref{sec:diversity_search}, each of which is in turn
an objective function or constraint used in our formulation
PMPS).

Regarding alternative approaches  -- we believe our learning based
Auto-Pipeline-RL (Section~\ref{sec:learning}) is 
a more principled alternative. Our hope is that it can learn
the intricate balance between these desirable dimensions, e.g. weighing
them appropriately, under different circumstances and
for different partial pipelines. We note that the 
learning based alternative also enjoys
the benefit of being more extensible to new desirable criteria that
one could decide to add into the formulation (beyond operator
probabilities, Key/FD, and column mappings currently exploited in our system).

We have updated our explanation and the running
example in \rev{Section~\ref{sec:diversity_search}} to 
make the intuition more clear.
%Another possible alternative here is to hand-tune a weighted function
%that combines the three dimensions into a single score, so that 
%we can come up with an overall top-K. 



\bigskip
\begin{tcolorbox}
\textbf{D12. “Because learning-based variants produce randomized results, we report numbers averaged over 5 runs” So how would one use your system in practice; run it multiple times until happy with the results?}
\end{tcolorbox}

\stitle{Response.}
We believe this 
is a confusion caused by our presentation. Like most machine learning
systems today, the RL variant of 
our algorithm is trained using standard stochastic gradient descent,
using randomized mini-batches of data points. 
As a result, running the offline training process $K$ times with
different initial seeds will lead
to $K$ slightly different models, as is typical in most ML models. 
However, once the model is trained offline, \textit{online prediction is 
deterministic for a given task},
such that the top-K synthesized pipelines returned by the learned
system is always identical, irrespective of how many times
users click on that ``synthesize'' button.
(An analogy here is that searching using the same query 
on Google $K$ times should lead to the same top-K results,
but if Google's ranking algorithm were trained using a 
different set of hyper-parameters and random seeds, the
results one would see for the same query may be slightly different).

In order to make sure that our superior results are not due to lucky
choices of random seeds, 
we average our results over 5 \textit{offline training runs} using different
seeds (and not over 5 online prediction runs).
This smooths out the randomness in 
the training process (inherent in stochastic gradient descent
and most other ML systems).
Our results suggest that the RL variant of our
algorithm consistently outperforms
previous baselines.  We have clarified this aspect 
in \rev{Section~\ref{sec:experiments}}
of our paper.



\bigskip
\begin{tcolorbox}
\textbf{D13. The results between Auto-pipeline-Search and -RL are quite close in Github (are they statistically significant?) but different in Commercial, more discussion is need on why this is the case and how the types of data would impact the proposed approach.}
\end{tcolorbox}

\stitle{Response.}
This is a great point. We performed paired t-tests, and found that
on the 700-case GitHub benchmarks, 
the advantage of
Auto-pipeline-RL over Auto-pipeline-Search 
on MRR is statistically significant (with p-value at 0.03).
However, the same advantage on accuracy 
is not statistically significant at p=0.05 level.

Perhaps surprisingly, even though the observed benefit
appears large on the Commercial benchmark, 
statistical tests show that the benefit is
actually not statistically significant for either MRR or Accuracy.
This is because this benchmark has only 16 pipelines
that we manually collected from tutorial materials of commercial
vendors (compared to the GitHub benchmark 
that has 700 pipelines automatically harvested online), limiting
the statistical power of tests run on this small set of test cases.
In the end, despite the seemingly strong benefit observed
in Table~\ref{tab:overall-commercial},
we could not actually draw reliable statistical conclusion
on this benchmark.

(It should be noted that during revision, we have tried to revisit this Commercial
benchmark to see if we could collect more test pipelines following
the same procedure. Unfortunately, despite our best effort,
we could find only a limited number of 
official tutorials for each of the vendors, limiting the
total number of test cases we can manually collect for this benchmark.)

\begin{comment}
\begin{table}
\centering
    \caption{P-value comparison }
    \vspace{-3mm}
    \label{tab:overall-github}
\begin{small}
\begin{tabular}{lrr}
        RL vs. Search & Accuracy & MRR   \\
        \midrule
        \sjs   & 76.6\%     & 0.724   \\
        \midrule
        \sjsl  & 73.7\%     & 0.583   \\
        \midrule
        \sjrl  & \textbf{76.9\%}     & \textbf{0.738} 
    \end{tabular}
\end{small}
\end{table}
\end{comment}

Overall, we believe these comparisons 
perhaps points to two explanations: (1) our hand-designed
and manually-tuned search strategy using diversity
(in Section~\ref{sec:diversity_search})
for Auto-pipeline-Search is already reasonably effective in synthesizing
data pipelines, making the benefit of Auto-pipeline-RL 
over Auto-pipeline-Search
less significant; and (2) while the benefit of 
Auto-pipeline-RL over Auto-pipeline-Search is somewhat mixed
(e.g., statistically significant for MRR not but for Accuracy),
it nevertheless takes away the
burden of hand-crafting search strategies tailored to our synthesis task, 
making the RL-based approach easier to generalize to new
operators that we may want to add to our DSL, and new
constraints that we may want to leverage in formulating the 
PMPS problem. 

We added these discussions in \rev{Section~\ref{sec:experiments}}
of our paper as suggested.

\bigskip
\begin{tcolorbox}
\textbf{D14. Other comments: 
\\
a. “reaching $10^{20}$ within 5 steps on typical tables” how was this figure obtained?
\\
b-d. Sentences to rephrase.}
\end{tcolorbox}


\stitle{Response.}
a. “reaching $10^{20}$ within 5 steps on typical tables”  -- this is based on the calculation that when given two 10-column tables, naively enumerating
even one step for all possible join-paths (assuming up to two
columns can join), would require enumerating $O(10^2)$ column-pairs
for one table, and $O(10^4)$ for both tables. (Similarly,
a 3-column group-by and 1-column aggregation on a 10-column
table would also lead to $O(10^4)$ possible options on one table). 
With join/group-by only 
and without considering other operators, a 5-step pipeline
would already translate to $O(10^4)^5 = 10^{20}$ total options, thus
the result. We have added a brief explanation of this calculation in 
\rev{Section~\ref{sec:intro}} of our revised paper.


b-d. We have fixed these issues and we thank the reviewer for pointing them out.
